Principal Bit Analysis: Autoencoding with Schur-Concave Loss

We consider a linear autoencoder in which the latent variables are quantized, or corrupted by noise, and the constraint is Schur-concave in the set of latent variances. Although finding the optimal encoder/decoder pair for this setup is a nonconvex optimization problem, we show that decomposing the source into its principal components is optimal. If the constraint is strictly Schur-concave and the empirical covariance matrix has only simple eigenvalues, then any optimal encoder/decoder must decompose the source in this way. As one application, we consider a strictly Schur-concave constraint that estimates the number of bits needed to represent the latent variables under fixed-rate encoding, a setup that we call \emph{Principal Bit Analysis (PBA)}. This yields a practical, general-purpose, fixed-rate compressor that outperforms existing algorithms. As a second application, we show that a prototypical autoencoder-based variable-rate compressor is guaranteed to decompose the source into its principal components.

==> pba-tex 2/abstract.tex <==
\begin{abstract}
%    We consider a linear autoencoder in which the latent variables
%    are corrupted by noise and the constraint
%    is Schur concave in the set of latent variances.
%    Although finding the optimal encoder/decoder pair 
%    for this autoencoder is a nonconvex optimization problem, we show that 
%    decomposing the source into its principal components is optimal, and 
%    if the constraint is strictly Schur concave, then any optimal
%    solution must decompose the source in this way.
%     We consider in particular a strictly Schur
%    concave constraint that estimates the number of bits needed to
%    represent the latent variables under fixed-rate encoding, which
%    we call \emph{Principal Bit Analysis (PBA)} and a generalization
%    that we call \emph{Principal Bit/Component Analysis (PBCA).} The
%    solution of these special cases yields an algorithm that unifies
%    Principal Components Analysis (PCA) and the reverse-waterfilling 
%    procedure from rate-distortion theory. It also yields a practical,
%    general-purpose, fixed-rate compressor that outperforms 
%    existing algorithms.
We consider a linear autoencoder in which the latent variables
    are quantized, or corrupted by noise, and the constraint
    is Schur-concave in the set of latent variances.
    Although finding the optimal encoder/decoder pair 
    for this setup is a nonconvex optimization problem, we show that 
    decomposing the source into its principal components is optimal. If 
    the constraint is strictly Schur-concave and the empirical
	  covariance matrix has only simple eigenvalues, then any optimal
	  encoder/decoder must decompose the source in this way. As one application,
     we consider a strictly Schur-concave constraint that estimates the 
      number of bits needed to represent the latent variables under 
      fixed-rate encoding, a setup that
    we call \emph{Principal Bit Analysis (PBA)}.  This yields a practical,
    general-purpose, fixed-rate compressor that outperforms 
    existing algorithms. As a second application, we show that a
      prototypical autoencoder-based variable-rate compressor is guaranteed
	  to decompose the source into its principal components.
	  
	  
\end{abstract}





==> pba-tex 2/experiments.tex <==
\section{Compression Experiments}\label{sec:EXPERIMENTS}

We validate the PBA algorithm experimentally by comparing the performance
of a PBA-derived fixed-rate compressor against  the performance of baseline fixed-rate
compressors. The code of our implementation can be found at \url{https://github.com/SourbhBh/PBA}. As we noted in the previous section, although variable-rate codes are more commonplace in practice, fixed-rate codes do offer some advantages over their more
general counterparts:
\begin{enumerate}
    \item In applications where a train of source
        realizations are compressed sequentially, fixed-rated 
        coding allows for simple concatenation of the compressed
        representations. Maintaining synchrony between the encoder
        and decoder is simpler than with variable-rate codes.
    \item In applications where a dataset of source realizations
        are individually compressed, fixed-rate coding allows for random access
        of data points from the compressed representation.
    \item In streaming in which a sequence of realizations will 
           be streamed, bandwidth provisioning is 
        simplified when the bit-rate is constant over time.
\end{enumerate}
% A \emph{fixed-rate} code for a random $d$-dimensional
%vector consists of an encoder 
%$$
%f : \mathbb{R}^d \mapsto \{0,1\}^R
%$$
%and a decoder
%$$
%g : \{0,1\}^R \mapsto \mathbb{R}^d, 
%$$
%
%where $R$ is an integer describing the \emph{rate} of the code,
%which is one figure of merit, the other being the expected
%distortion between the source $X$ and the reconstruction
%$g(f(X))$. For comparison, a \emph{variable-rate} code 
%consists of an encoder/decoder pair
%\begin{align}
%    f & : \mathbb{R}^d \mapsto \{0,1\}^* \\
%    g & : \{0,1\}^* \mapsto \mathbb{R}^d, 
%\end{align}
%with the rate defined as $E[\ell(f(X))]$, where $\ell(b)$ denotes
%the length of the binary string $b$. 
%
%Evidently fixed-rate codes are a special case of variable-rate
%codes, and thus any performance that is achievable with the
%former is also achievable with the latter. Indeed, most
%practical multimedia compression algorithms are variable-rate~\cite{??}
%and recent applications of autoencoders to multimedia compression
%are also variable rate~\cite{??}.
%Fixed-rate codes do offer some advantages over their more
%general counterparts, however:
%\begin{enumerate}
%    \item In applications in which a train of source
%        realizations will be compressed sequentially, fixed-rated 
%        coding allows for simple concatenation of the compressed
%        representations. Maintaining synchrony between the encoder
%        and decoder is simpler than with variable-rate codes.
%    \item In applications in which a dataset of source realizations
%        are individually compressed, fixed-rate coding allows for random access
%        of the data points from the compressed representation.
%    \item In streaming in which a sequence of realizations will 
%           be streamed, bandwidth provisioning is 
%        simplified when the bit-rate is constant over time.
%\end{enumerate}

Fixed-rate compressors exist for specialized sources such as
speech~\cite{McCreeB95, SchroederA85} and audio more 
generally~\cite{Vorbis}. We
consider a general-purpose, learned, fixed-rate compressor
derived from PBA and the following two quantization operations.
The first, $Q_{CD}(a,\sigma^2,U,x)$\footnote{``CD'' stands for 
``clamped dithered.''}
accepts the hyperparameter $a$, a variance estimate $\sigma^2$, a
dither realization $U$, and the scalar source realization to be
compressed, $x$, and outputs (a binary representation of) the
nearest point to $x$ in the set
% TODO: confirm this is the same as dithered quantization
\begin{equation}
    \label{eq:quantizeset}
    \left\{i + U : i \in \mathbb{Z} \ \text{and} \ i + U 
         \in \left(-\frac{\Gamma}{2},\frac{\Gamma}{2}\right] \right\}\newest{,}
\end{equation}
where
\begin{equation}
    \Gamma = 2^{\lfloor \frac{1}{2} \log_2 (4a^2 \sigma^2 + 1) \rfloor }.
\end{equation}
% TODO: what is the convention for the base of logarithms?
This evidently requires $\log_2 \Gamma$ bits.  The second
function, $Q_{CD}'(a^2,\sigma^2,U,b)$, where $b$ is a binary
string of length $\log_2 \Gamma$, maps the binary
representation $b$ to the point in~(\ref{eq:quantizeset}).
These quantization routines are applied separately to each
latent component. The $\sigma^2$ parameters are
determined during training. The dither $U$ is chosen
uniformly over the set $[-1/2,1/2]$, independently for
each component. We assume that $U$ is chosen pseudorandomly
from a fixed seed that is known to both the encoder and
the decoder. As such, it does not need to be explicitly 
communicated. For our experiments, we fix the $a$ parameter
at $15$ and hard code this both at the encoder and at
the decoder. We found that this choice balances the 
dual goals of minimizing the excess distortion due to 
the clamping quantized points to the interval $(\Gamma/2,\Gamma/2]$ 
and minimizing the rate.

PBA compression proceeds by applying Algorithm~\ref{alg:PBA}
to a training set to determine the matrices $\encnew$ and 
$\decnew$. The variance estimates $\sigma_1^2,\ldots,\sigma_d^2$
for the $d$ latent variances are chosen as the empirical 
variances on the training set and are hard-coded in the encoder
and decoder. Given a data point $\data$,
the encoded representation is the concatenation of the bit strings
$b_1, \ldots, b_d$, where
$$
b_i = Q_{CD}(a^2,\sigma^2_i,U_i,\encvec_i^\top x), 
$$ 
% TODO: need to define U_1. Only U is defined above.
The decoder parses the received bits into $b_1, \ldots, b_d$. 
and computes the latent reconstruction $\hat\latent$, where
$$
\hat\latent_i = Q_{CD}'(a^2,\sigma^2_i,U_i,b_i), 
$$
The reconstruction is then $\decnew\hat\latent$. 

We evaluate the PBA compressor on MNIST \cite{LecunBBH98}, CIFAR-10 \cite{Krizhevsky09}, MIT Faces Dataset, Free Spoken Digit Dataset (FSDD) \cite{Zohar} and a synthetic Gaussian dataset. The synthetic Gaussian dataset is generated from a diagonal covariance matrix obtained from the eigenvalues of the Faces Dataset. 
We compare our algorithms primarily using mean-squared error since our theoretical analysis uses mean squared error as the distortion metric. Our plots display Signal-to-Noise ratios (SNRs) for ease of interpretation. For image datasets, we also compare our algorithms using the Structural Similarity (SSIM) or the Multi-scale Strctural Similarity (MS-SSIM) metrics when applicable \cite{WangBSS04}. We also consider errors on downstream tasks, specifically classification, as a distortion measure.

For all datasets, we compare the performance of the PBA compressor 
against baseline scheme derived from PCA that uses $Q_{CD}$
and $Q_{CD}'$.
The PCA-based scheme sends some of the principal components 
essentially losslessly, and no information about the others.
Specifically, in the context of our framework,
for any given $k$, we choose the first $k$ columns
of $\encnew$ to be aligned with the first $k$ principal components
of the dataset; the remaining columns are zero. Each nonzero column
is scaled such that its Euclidean length multiplied by the eigenvalue has all the significant digits. This is done so that at high rates, the quantization procedure sends the $k$ principal components losslessly. The quantization
and decoder operations are as in the PBA-based scheme; in particular
the $a^2$ parameter is as specified above. By varying $k$, we trade off rate and distortion. 

%For image datasets we also compare against JPEG and JPEG2000, which are standard variable-rate compression schemes. For audio datasets,
%we also compare against AAC, a standard fixed-rate compression
%scheme.

% TODO: rounding vs. nonrounding of image pixsels
% TODO: plot theoretical predicrtion

% TODO: emphasize that we use the same quantization scheme with both
% PBA and PCA to be fair.

% TODO: literature search on learned, fixed-rate compression

\subsection{SNR Performance}
%\begin{figure}[H]
%\minipage{0.32\textwidth}
%  \includegraphics[width=\linewidth]{images/MNIST_MSE_PBAPCAJPEG.png}
%  %\caption{MNIST}\label{fig:mnist_mse}
%\endminipage\hfill
%\minipage{0.32\textwidth}
%  \includegraphics[width=\linewidth]{images/CIFAR_MSE_PBAPCAJPEG.png}
% % \caption{CIFAR-10}\label{fig:cifar_mse}
%\endminipage\hfill
%\minipage{0.32\textwidth}%
%  \includegraphics[width=\linewidth]{images/FACES_MSE_PBAPCAJPEG.png}
%%  \caption{Faces dataset}\label{fig:faces_mse}
%\endminipage \hfill
%\minipage{0.32\textwidth}
%  \includegraphics[width=\linewidth]{images/MNIST_MSE_PBAPCAJPEG_zoom.png}
%  %\caption{MNIST}\label{fig:mnist_mse}
%\endminipage\hfill
%\minipage{0.32\textwidth}
%  \includegraphics[width=\linewidth]{images/CIFAR_MSE_PBAPCAJPEG_zoom.png}
% % \caption{CIFAR-10}\label{fig:cifar_mse}
%\endminipage\hfill
%\minipage{0.32\textwidth}%
%  \includegraphics[width=\linewidth]{images/FACES_MSE_PBAPCAJPEG_zoom.png}
%%  \caption{Faces dataset}\label{fig:faces_mse}
%\endminipage \hfill
%\minipage{0.32\textwidth}
%  \includegraphics[width=\linewidth]{images/MNIST_MSE_PBAPCAJPEG_UltraZoom.png}
%  %\caption{MNIST}\label{fig:mnist_mse}
%\endminipage\hfill
%\minipage{0.32\textwidth}
%  \includegraphics[width=\linewidth]{images/CIFAR_MSE_PBAPCA_UltraZoom.png}
% % \caption{CIFAR-10}\label{fig:cifar_mse}
%\endminipage\hfill
%\minipage{0.32\textwidth}%
%  \includegraphics[width=\linewidth]{images/FACES_MSE_PBAPCAJPEG_UltraZoom.png}
%%  \caption{Faces dataset}\label{fig:faces_mse}
%\endminipage
%\centering
%\caption{MSE/pixel vs Rate (bits/pixel) for MNIST, CIFAR-10, Faces Dataset. Figures at the bottom are progressively zoomed-in. }\label{fig:mse}
%\end{figure}




\begin{figure}[hbt]
\centering
\minipage{0.18\textwidth}
  \includegraphics[width=\linewidth]{images/Reconstructions_PCA_1.png}
  %\caption{MNIST}\label{fig:mnist_mse}
\endminipage\hfill
\minipage{0.18\textwidth}
  \includegraphics[width=\linewidth]{images/Reconstructions_PCA_2.png}
  %\caption{MNIST}\label{fig:mnist_mse}
\endminipage\hfill
\minipage{0.18\textwidth}
  \includegraphics[width=\linewidth]{images/Reconstructions_PCA_3.png}
  %\caption{MNIST}\label{fig:mnist_mse}
\endminipage\hfill
\minipage{0.18\textwidth}
  \includegraphics[width=\linewidth]{images/Reconstructions_PCA_4.png}
  %\caption{MNIST}\label{fig:mnist_mse}
\endminipage\hfill
\minipage{0.18\textwidth}
  \includegraphics[width=\linewidth]{images/Reconstructions_PCA_5.png}
  %\caption{MNIST}\label{fig:mnist_mse}
\endminipage\hfill 
\minipage{0.18\textwidth}
  \includegraphics[width=\linewidth]{images/Reconstructions_PBA_1.png}
  %\caption{MNIST}\label{fig:mnist_mse}
\endminipage\hfill
\minipage{0.18\textwidth}
  \includegraphics[width=\linewidth]{images/Reconstructions_PBA_2.png}
  %\caption{MNIST}\label{fig:mnist_mse}
\endminipage\hfill
\minipage{0.18\textwidth}
  \includegraphics[width=\linewidth]{images/Reconstructions_PBA_3.png}
  %\caption{MNIST}\label{fig:mnist_mse}
\endminipage\hfill
\minipage{0.18\textwidth}
  \includegraphics[width=\linewidth]{images/Reconstructions_PBA_4.png}
  %\caption{MNIST}\label{fig:mnist_mse}
\endminipage\hfill
\minipage{0.18\textwidth}
  \includegraphics[width=\linewidth]{images/Reconstructions_PBA_5.png}
  %\caption{MNIST}\label{fig:mnist_mse}
\endminipage\hfill
\caption{Reconstructions at different bits/pixel values for PCA (top) and PBA (bottom)}\label{fig:reconstructions_pca_pba}
\end{figure}


\begin{figure}[hbt]
\centering
\minipage{0.24\textwidth}
  \includegraphics[width=\linewidth]{images/MNIST_SNR_PBAPCAJPEG.png}
  %\caption{MNIST}\label{fig:mnist_mse}
\endminipage\hfill
\minipage{0.24\textwidth}
  \includegraphics[width=\linewidth]{images/CIFAR_SNR_PBAPCAJPEG.png}
 % \caption{CIFAR-10}\label{fig:cifar_mse}
\endminipage\hfill
\minipage{0.24\textwidth}%
  \includegraphics[width=\linewidth]{images/FACES_SNR_PBAPCAJPEG.png}
%  \caption{Faces dataset}\label{fig:faces_mse}
\endminipage \hfill
\minipage{0.24\textwidth}%
  \includegraphics[width=\linewidth]{images/AUDIO_SNR.png}
%  \caption{Faces dataset}\label{fig:faces_mse}
\endminipage \hfill
\minipage{0.24\textwidth}
  \includegraphics[width=\linewidth]{images/MNIST_SNR_PBAPCAJPEG_UltraZoom.png}
  %\caption{MNIST}\label{fig:mnist_mse}
\endminipage\hfill
\minipage{0.24\textwidth}
  \includegraphics[width=\linewidth]{images/CIFAR_SNR_PBAPCA_UltraZoom.png}
 % \caption{CIFAR-10}\label{fig:cifar_mse}
\endminipage\hfill
\minipage{0.24\textwidth}%
  \includegraphics[width=\linewidth]{images/FACES_SNR_PBAPCAJPEG_UltraZoom.png}
  \endminipage \hfill
  \minipage{0.24\textwidth}%
  \includegraphics[width=\linewidth]{images/AUDIO_SNR_Zoom.png}
%  \caption{Faces dataset}\label{fig:faces_mse}

%  \caption{Faces dataset}\label{fig:faces_mse}
\endminipage
\caption{SNR/pixel vs Rate (bits/pixel) for MNIST, CIFAR-10, Faces, FSDD datasets. Figures in the bottom row are zoomed-in. } \label{fig:snr}
   
\end{figure}

\begin{figure}[hbt]
\centering
\minipage{0.24\textwidth}
  \includegraphics[width=\linewidth]{images/MNIST_NQ_SNR_PBAPCA.png}
  %\caption{MNIST}\label{fig:mnist_mse}
\endminipage\hfill
\minipage{0.24\textwidth}
  \includegraphics[width=\linewidth]{images/CIFAR_NQ_SNR_PBAPCA.png}
 % \caption{CIFAR-10}\label{fig:cifar_mse}
\endminipage\hfill
\minipage{0.24\textwidth}%
  \includegraphics[width=\linewidth]{images/FACES_NQ_SNR_PBAPCA.png}
  
%  \caption{Faces dataset}\label{fig:faces_mse}
\endminipage
\minipage{0.24\textwidth}%
  \includegraphics[width=\linewidth]{images/SYN_PBA_PCA.png}
  
%  \caption{Faces dataset}\label{fig:faces_mse}
\endminipage


\minipage{0.24\textwidth}
  \includegraphics[width=\linewidth]{images/MNIST_NQ_SNR_PBAPCA_UltraZoom.png}
  %\caption{MNIST}\label{fig:mnist_mse}
\endminipage\hfill
\minipage{0.24\textwidth}
  \includegraphics[width=\linewidth]{images/CIFAR_NQ_SNR_PBAPCA_UltraZoom.png}
 % \caption{CIFAR-10}\label{fig:cifar_mse}
\endminipage\hfill
\minipage{0.24\textwidth}%
  \includegraphics[width=\linewidth]{images/FACES_NQ_SNR_PBAPCA_UltraZoom.png}
  
%  \caption{Faces dataset}\label{fig:faces_mse}
\endminipage
\minipage{0.24\textwidth}%
  \includegraphics[width=\linewidth]{images/SYN_PBA_ULTRAZOOM.png}
  
%  \caption{Faces dataset}\label{fig:faces_mse}
\endminipage


\caption{SNR/pixel vs Rate (bits/pixel) for MNIST, CIFAR-10, Faces and Synthetic dataset. Reconstructions are not rounded to integers from $0$ to $255$. The bottom four plots are zoomed-in versions of the top four plots.}
\label{fig:nq}
\end{figure}


\begin{figure}[hbt]
\centering
\minipage{0.24\textwidth}
  \includegraphics[width=\linewidth]{images/MNIST_EIG_LARGEST.png}
  %\caption{MNIST}\label{fig:mnist_mse}
\endminipage\hfill
\minipage{0.24\textwidth}
  \includegraphics[width=\linewidth]{images/CIFAR_EIG_LARGEST.png}
 % \caption{CIFAR-10}\label{fig:cifar_mse}
\endminipage\hfill
\minipage{0.24\textwidth}%
  \includegraphics[width=\linewidth]{images/FACES_EIG_LARGEST.png}
\endminipage\hfill
\minipage{0.24\textwidth}%
  \includegraphics[width=\linewidth]{images/AUDIO_EIG_LARGEST.png}
  \endminipage
  
  
\minipage{0.24\textwidth}
  \includegraphics[width=\linewidth]{images/MNIST_EIG_SMALLEST.png}
  %\caption{MNIST}\label{fig:mnist_mse}
\endminipage\hfill
\minipage{0.24\textwidth}
  \includegraphics[width=\linewidth]{images/CIFAR_EIG_SMALLEST.png}
 % \caption{CIFAR-10}\label{fig:cifar_mse}
\endminipage\hfill
\minipage{0.24\textwidth}%
  \includegraphics[width=\linewidth]{images/FACES_EIG_SMALLEST.png}
%  \caption{Faces dataset}\label{fig:faces_mse}
\endminipage\hfill
\minipage{0.24\textwidth}%
  \includegraphics[width=\linewidth]{images/AUDIO_EIG_SMALLEST.png}
  \endminipage
\caption{Eigenvalue distribution of the datasets. The top three plots are the largest 25 eigenvalues for MNIST, CIFAR-10, Faces and FSDD dataset. The bottom four figures plot the remaining eigenvalues except the largest 500. }
\label{fig:eig}
\end{figure}


\begin{figure}[hbt]
\centering
\minipage{0.32\textwidth}
  \includegraphics[width=\linewidth]{images/MNIST_COMP.png}
  %\caption{MNIST}\label{fig:mnist_mse}
\endminipage\hfill
\minipage{0.32\textwidth}
  \includegraphics[width=\linewidth]{images/CIFAR_COMP.png}
 % \caption{CIFAR-10}\label{fig:cifar_mse}
\endminipage\hfill
\minipage{0.32\textwidth}%
  \includegraphics[width=\linewidth]{images/FACES_COMP.png}
\endminipage
\caption{Plots of number of components sent vs rate (bits/pixel) for PBA and PCA. }\label{fig:num_comp}
\end{figure}

We begin by examining compression performance under
mean squared error, or equivalently, the SNR, defined as
$$
\text{SNR} = 10 \cdot \log_{10}\left( 
                \frac{P}{\text{MSE}}\right).
$$
where $P$ is the empirical second moment of the dataset.
% TODO: empirical second moment vs. empirical variance
This was the objective that PBA (and PCA) is designed to minimize.

%Figure~\ref{fig:snr-theory} shows the rate-SNR tradeoff for the PBA
%and PCA compressors and the tradeoff obtained from the solution 
%to~(\ref{fig:nq}). 
%COMMENT ON SIMILARITY. We see that PBA consistently outperforms PCA
%by a significant margin, indicating that while PCA is useful for
%dimensionality reduction, it makes for a crude compression 
%technique.\footnote{See~\cite{??} for works that explicitly employ
%PCA as a compression method.}
%Ask Aaron 

In Figure~\ref{fig:reconstructions_pca_pba}, we display reconstructions 
for a particular image in the Faces Dataset under PBA and PCA.
Figure~\ref{fig:snr} shows the tradeoff for PBA and PCA against
JPEG and JPEG2000 (for the image datasets) and 
AAC (for the audio dataset). All of the image datasets
have integer pixel values between 0 and 255. Accordingly, we round
the reconstuctions of PBA and PCA to the nearest integer in this range. Figure~\ref{fig:nq} shows the same tradeoff for PBA and PCA when reconstructions are not rounded off to the nearest integer.
We see that PBA consistently
outperforms PCA and JPEG, and is competitive with JPEG2000, even 
though the JPEG and JPEG2000 are variable-rate.  \footnote{It should be 
noted, however, that JPEG and JPEG2000 aim to minimize subjective
distortion, not MSE, and they 
do not allow for training on sample images, as PBA and PCA do. A
similar caveat applies to AAC.} We estimate the size of the JPEG header by compressing an empty image and subtract this estimate from all the compression sizes produced by JPEG. We do not plot JPEG2000 performance for MNIST since it requires at least a 32x32 image. For audio data, we observe that PBA consistently outperforms PCA and AAC.
Since the image data all use $8$ bits per pixel, one can 
obtain infinite SNR at this rate via the trivial encoding that
communicates the raw bits. PCA and PBA do not find this solution
because they quantize in the transform domain, where the
lattice-nature of the pixel distribution is not apparent.
Determining how to leverage lattice structure in the source
distribution for purposes of compression is an interesting
question that transcends the PBA and PCA algorithms and that
we will not pursue here.

The reason that PCA performs poorly is that it 
favors sending the less significant bits of the most significant 
components over the most significant bits of less significant 
components, when the latter are more valuable for reconstructing
the source.  Arguably, it does not identify the ``principal bits.''
Figure~\ref{fig:eig} shows the eigenvalue distribution of the 
different datasets, and Figure~\ref{fig:num_comp} shows the number of distinct
components about which information is sent as a function of rate
for both PBA and PCA. We see that PBA sends information about many 
more components for a given rate than does PCA. We discuss the
ramifications of this for downstream tasks, such as classification,
in Section~\ref{subsec:downstream}.

% TODO: confirm image datasets all use 8 bits per pixel and are gray scale.





%\begin{figure}[!htb]
%\includegraphics[width=0.5\textwidth]{images/SYN_GAUSSIAN_PBAPCA.png}
%\caption{MSE per pixel vs Rate(bpp) for Synthetic Gaussian Dataset}
%\end{figure}





%We expect more uniform eigenvalue distributions to expose a larger
%gap between PCA and PBA. In the extreme case of a uniform eigenvalue
%distribution, PBA will send information about as many components
%as possible, while PCA will send information about as few as possible.
%To confirm this experimentally, we make the eigenvalues of the Faces dataset successively more uniform by adding salt and pepper noise. Salt and pepper noise with $p$ probability of corruption is obtained by making a randomly selected  $p/2$-fraction of pixels equal to $0$ (white) and a  randomly selected $p/2$-fraction of the pixels equal to $255$ (black). Figure~\ref{fig:saltpepper_eig} illustrates the successive uniform eigenvalues as the probability is increased.
%\begin{figure}[hbt!]
%\minipage{0.47\textwidth}
%  \includegraphics[width=\linewidth]{images/SP_EIG_SMALLEST.png}
%  %\caption{MNIST}\label{fig:mnist_mse}
%\endminipage\hfill
%\minipage{0.47\textwidth}
%  \includegraphics[width=\linewidth]{images/SP_EIG_LARGEST.png}
% % \caption{CIFAR-10}\label{fig:cifar_mse}
%\endminipage
%\centering
%\caption{Eigenvalues of the Faces Dataset with and without noise}\label{fig:saltpepper_eig}
%\end{figure}

%Figure~\ref{fig:saltpepper_mse} shows that PBA outperforms PCA by a larger margin after the addition of salt and pepper noise. 
%
%\begin{figure}[hbt!]
%\minipage{0.47\textwidth}
%  \includegraphics[width=\linewidth]{images/SP_MSE_no1020.png}
%  %\caption{MNIST}\label{fig:mnist_mse}
%\endminipage\hfill
%\minipage{0.47\textwidth}
%  \includegraphics[width=\linewidth]{images/SP_NQ_no1020.png}
% % \caption{CIFAR-10}\label{fig:cifar_mse}
%\endminipage
%\centering
%\caption{MSE/pixel vs Rate (Bits/pixel) : Quantized and Non-Quantized}\label{fig:saltpepper_mse}
%\end{figure}


\subsection{SSIM Performance}

Structural similarity (SSIM) and Multi-Scale Structural similarity (MS-SSIM) are metrics that are tuned to perceptual similarity. Given two images, the SSIM metric outputs a real value between $0$ and $1$ where a higher value indicates more similarity between the images. We evaluate the performance of our algorithms on these metrics as well in Figure~\ref{fig:ssim}. We see that PBA
consistently dominates PCA, and although it was not optimized for
this metric, beats JPEG at low rates as well.

\begin{figure}[hbt]
\centering
\minipage{0.32\textwidth}
  \includegraphics[width=\linewidth]{images/MNIST_SSIM_PBAPCAJPEG.png}
  %\caption{MNIST}\label{fig:mnist_mse}
\endminipage\hfill
\minipage{0.32\textwidth}
  \includegraphics[width=\linewidth]{images/CIFAR_SSIM_PBAPCAJPEG.png}
 % \caption{CIFAR-10}\label{fig:cifar_mse}
\endminipage\hfill
\minipage{0.32\textwidth}%
  \includegraphics[width=\linewidth]{images/FACES_SSIM_PBAPCAJPEG.png}
%  \caption{Faces dataset}\label{fig:faces_mse}
\endminipage
\caption{SSIM vs Rate (bits/pixel) for MNIST, CIFAR-10, Faces Dataset}\label{fig:ssim}
\end{figure}

%
%\subsection{Performance of PBCA}
%To examine the empirical performance of PBCA we use the synthetic dataset. We also fix $\scalePBA=1$ and instead adjust the scaling of $\scale$ appropriately.  We study the performance of PBCA in two ways. The first aims at verifying an improvement over PBA by comparing performance for different values of $\scale$. The second aims at verifying convergence to PCA according to Theorem~\ref{thm:PBCA-PCA}. We plot the performance without rounding, in all figures since rounding is an additional nonlinear transformation.
%
%%Each curve in Figure~\ref{fig:pbca_pba} is generated by running PBCA over different rates for a fixed value of $\scale$. Note that $\scale=0$ is outperformed by values of $\scale$ that are larger than 0, except $\scale =100$ although the difference does not appear to be large on a semilogy plot. This suggests a trend where the performance is optimal for some intermediate value of $\scale$. In our implementation, we estimate the overhead per pixel to be around 1.27 bits. This value of $\scale$ is optimal among the $\scale$ curves we plotted. 
%
%To verify convergence of PBCA to PCA as proven in Theorem~\ref{thm:PBCA-PCA},for a fixed $\scale$ we run PBCA with rate $k\scale + m$ for $k=3500$. As the value of $\scale$ increases, we observe from Figure~\ref{fig:pbca_pca} that the distortion approaches that of PCA. Although Theorem~\ref{thm:PBCA-PCA} requires $\scalePBA \rightarrow 0$, $\scale \rightarrow \infty$ is equivalent. 
%
%
%In Figure~\ref{fig:pbca_pba}, we plot the distortion of PBCA for a fixed rate - 2.9006 bits/pixel versus $\scale$. This shows that if PBCA is constrained to send only ~3 bits/pixel, setting $\scale=0$, which is PBA, is not optimal. In addition, an intermediate value of $\scale$, which is closer to the estimated overhead, is optimal. 
%
%
%\begin{figure}[hbt!]
%\minipage{0.45\textwidth}
%  \includegraphics[width=\linewidth]{images/SYN_PBCA_PCA.png}
%  \caption{MSE/pixel vs Rate(bits/pixel) for PBCA to show convergence to PCA for a Synthetic Dataset}\label{fig:pbca_pca}
%\endminipage\hfill
%\minipage{0.45\textwidth}
%  \includegraphics[width=\linewidth]{images/SYN_PBCA_PBA.png}
%  \caption{MSE/pixel vs Rate(bits/pixel) for PBCA to show effect of $\scale$ on performance, for a Synthetic Dataset}\label{fig:pbca_pba}
%\endminipage\hfill
%\centering
%\end{figure}

\subsection{Performance on Downstream tasks}
\label{subsec:downstream}
Lastly, we compare the impact of using PBA and PCA on an important downstream task, namely classification. We evaluate the algorithms on MNIST and CIFAR-10 datasets and use neural networks for classification. Our hyperparameter and architecture choices are given in Table~\ref{tb:ARCHITECTURE}. We divide the dataset into three parts. From the first part, we obain the covariance matrix that we use for PCA and to obtain the PBA compressor. The second and third part are used as training and testing data for the purpose of classification. For a fixed rate, reconstructions are passed to the neural networks for training and testing respectively. Since our goal is to compare classification accuracy across the compressors, we fix both the architecture and hyperparameters, and do not perform any additional tuning for the separate algorithms.


Figure~\ref{fig:accuracy} shows that PBA outperforms PCA in terms of accuracy. The difference is especially significant for low rates; all algorithms attain roughly the same performance at higher rates.

%TODO: mention that complexity increases with dimension, which is a 
% reason to use PCA or PBCA.

%\begin{figure}[!htb]
\begin{table}[hbt]
\centering

\begin{tabular}[t]{lccc}
\hline
Hyperparameter&MNIST&CIFAR-10\\
\hline
Architecture & 2-layer fully connected NN & Convolutional Neural Network \\ & & with 2 convolutional layers, pooling and \\ & & three fully connected layers \\
\# Hidden Neurons&100& NA\\
Optimization Algorithm&Adam& SGD with momentum\\
Loss&Cross-entropy&Cross-entropy\\
Learning Rate&0.0005&0.01\\
\hline
\end{tabular}
\caption{Hyperparameter Choices and Architecture for Classification}\label{tb:ARCHITECTURE}
\end{table}%

\begin{figure}[hbt]
\centering
\minipage{0.45\textwidth}
  \includegraphics[width=\linewidth]{images/CIFAR_ACCURACY_PBAPCAJPEG.png}
  %\caption{MNIST}\label{fig:mnist_mse}
\endminipage\hfill
\minipage{0.45\textwidth}
  \includegraphics[width=\linewidth]{images/MNIST_ACCURACY_PBAPCAJPEG.png}
 % \caption{CIFAR-10}\label{fig:cifar_mse}
\endminipage
\caption{Accuracy vs Rate (bits/pixel) for MNIST, CIFAR-10}\label{fig:accuracy}
\end{figure}

%\begin{figure}[!htb]
%\centering
%\includegraphics[width=0.4\textwidth]{images/MNIST_ACCURACY_PBAPCAJPEG.png}
%\caption{Accuracy vs Rate(bpp) for MNIST}\label{fig:mnist_accuracy}
%\end{figure}
%\centering
%\includegraphics[width=0.4\textwidth]{images/SP_EIG.png}
%\caption{Eigenvalues of the Faces Dataset with and without noise. The top 500 eigenvalues are omitted to obtain a trend}\label{fig:saltpepper_eig}
%\end{figure}

%\subsection{MIT Faces}
%We compare PCA and PBA on the Eigenfaces dataset (https://courses.media.mit.edu/2004fall/mas622j/04.projects/faces/) that has 3993 images of dimension $128 \times 128$ pixels. The entire dataset, denoted by $X$ is stored in a $3993\times16384$  matrix which is then centered. The covariance matrix $K$ is a $16384 \times 16384$  matrix. 
%
%\subsubsection{PCA} 
%For a fixed number of components $c$, the top $c$ eigenvectors of $K$ are extracted and the dataset $X$ is projected onto the top $c$ eigenvectors giving a $3993 \times c$ projection matrix $P$. Since for every image we intend to store the projection, we compute the rate by computing how many bits are required to store an image's projection, averaged over the dataset.
%
%\subsubsection{PBA}
%The PBA algorithm requires obtaining all the eigenvectors and eigenvalues of the covariance matrix $K$. For a fixed value of the rate parameter, the PBA algorithm decides the number of components (eigenvectors) to send and how much "information" is to be sent along them. Here "information" stands for the amount of scaling applied to each eigenvector and is captured in the diagonal matrix $W'$. The encoding matrix $W$ is obtained from $W'$ by premultiplying the eigenvector matrix $W = UW'$. For each image $x_i$, $W^Tx_i$ is its projection. Therefore for the entire dataset $X$, we compute the rate by computing the number of bits required to store  $P = XW$.
%
%\subsubsection{Computing Rate and MSE} 
%We now explicitly mention our procedure to compute the rate for both PCA and PBA.
%\begin{itemize}
%\item \textbf{Count exact number of bits} 
%\begin{enumerate}
%\item Compute the number of bits required to store the integer part and the fractional part of each entry of $P$ in both cases. Divide the result by the number of samples to get the rate in bits per image. Figure~\ref{fig:PBAvsPCA_MSE_sizes} shows that PBA obtains a lower MSE than PCA. Figure~\ref{fig:PBAvsPCA_SSIM_sizes} shows that PBA outperforms PCA for lower rates with respect to the SSIM metric which is claimed to correlate better with perceptual similarity.
%
%\begin{figure}[H]\label{fig:PBAvsPCA_MSE_sizes}
%\centering
%\includegraphics{../image_dump/PBAvsPCA_MSE_actualsizes}
%\caption{MSE vs Rate comparison for PBA and PCA}
%\end{figure}
%
%\begin{figure}[H]\label{fig:PBAvsPCA_SSIM_sizes}
%\centering
%\includegraphics{../image_dump/PBAvsPCA_SSIM_actualsizes}
%\caption{SSIM vs Rate comparison for PBA and PCA}
%\end{figure}
%
%\bnote{This is not representative of the theory because PBA has a addition of noise phase which we did not consider while computing rate}
%\item In this method, we compute the PCA rate as before. For PBA, we incorporate the addition of noise by quantizing (dropping the fractional part) the matrix $P$. We reconstruct the images from the quantized $P$ and then compute the MSE. Figure~\ref{fig:PBAvsPCA_MSE_quant} shows that even in this case, PBA outperforms PCA for MSE
%
%\begin{figure}[H]\label{fig:PBAvsPCA_MSE_quant}
%\centering
%\includegraphics{../image_dump/PBAvsPCA_quantize_MSE}
%\caption{MSE vs Rate comparison for PBA and PCA}
%\end{figure}
%\bnote{This also might not be the best way to compute bits of $P$ : PBA theory states that we allocate same number of bits for each component. In this method, we allocate different bits for each entry of $P$}
%\end{enumerate}
%\item \textbf{Median bits allocation}
%
%\item \textbf{Zip} : In this method, we compress the projection matrices through a standard lossless compressor. For PCA, we use the projection matrix $P$ as it is. For PBA, we use the quantized projection matrix and compute the MSE with reconstructions from the quantized projection matrices. We observe that while comparing MSE, for low rates, PCA outperforms PBA whereas for higher rates, PBA outperforms PCA.
%
%\begin{figure}[H]\label{fig:PBAvsPCA_MSE_zip}
%\centering
%\includegraphics{../image_dump/PBAvsPCA_zip_MSE}
%\caption{MSE vs Rate comparison for PBA and PCA : Zip}
%\end{figure}
%
%%\begin{figure}[H]\label{fig:PBAvsPCA_SSIM_zip}
%%\centering
%%\includegraphics{../image_dump/PBAvsPCA_zip_SSIM}
%%\caption{SSIM vs Rate comparison for PBA and PCA}
%%\end{figure}
%
%\bnote{Since, we are using the same method for both PCA and PBA, the absolute sizes of the compressed versions are not relevant for comparison. However, it was observed that writing the matrix to a binary file and then compressing gives a larger absolute size as compared to saving using the savez-compressed function in numpy}
%\end{itemize}
%%\begin{figure}[H]
%%\centering
%%\includegraphics{../image_dump/PCA_MSE_Num_Comp}
%%\caption{MSE vs Number of Components in PCA}
%%\end{figure}
%%
%%\begin{figure}[H]
%%\centering
%%\includegraphics{../image_dump/PBA_MSE_Rate}
%%\caption{MSE vs Rate in PBA}
%%\end{figure}
%
%
%
%
%\begin{figure}[H]
%\minipage{0.16\textwidth}
%  \includegraphics[width=\linewidth]{../image_dump/Reconst_PBA_10}
%  %\caption{Rate 10 nats}\label{fig:awesome_image1}
%\endminipage\hfill
%\minipage{0.16\textwidth}
%  \includegraphics[width=\linewidth]{../image_dump/Reconst_PBA_33}
% % \caption{Rate 33 nats}\label{fig:awesome_image2}
%\endminipage\hfill
%\minipage{0.16\textwidth}%
%  \includegraphics[width=\linewidth]{../image_dump/Reconst_PBA_73}
%  %\caption{Rate 73 nats}\label{fig:awesome_image3}
%\endminipage\hfill
%\minipage{0.16\textwidth}
%  \includegraphics[width=\linewidth]{../image_dump/Reconst_PBA_530}
%  %\caption{Rate 530 nats}\label{fig:awesome_image2}
%\endminipage\hfill
%\minipage{0.16\textwidth}
%  \includegraphics[width=\linewidth]{../image_dump/Reconst_PBA_1172}
%  %\caption{Rate 1172 nats}\label{fig:awesome_image2}
%\endminipage\hfill
%\minipage{0.16\textwidth}
%  \includegraphics[width=\linewidth]{../image_dump/Original_Image}
%  %\caption{Original Image}\label{fig:awesome_image2}
%\endminipage\hfill
%\caption{PBA}
%\end{figure}
%
%
%\begin{figure}[H]
%\minipage{0.16\textwidth}
%  \includegraphics[width=\linewidth]{../image_dump/Reconst_PCA_1}
%  %\caption{Rate 10 nats}\label{fig:awesome_image1}
%\endminipage\hfill
%\minipage{0.16\textwidth}
%  \includegraphics[width=\linewidth]{../image_dump/Reconst_PCA_10}
% % \caption{Rate 33 nats}\label{fig:awesome_image2}
%\endminipage\hfill
%\minipage{0.16\textwidth}%
%  \includegraphics[width=\linewidth]{../image_dump/Reconst_PCA_50}
%  %\caption{Rate 73 nats}\label{fig:awesome_image3}
%\endminipage\hfill
%\minipage{0.16\textwidth}
%  \includegraphics[width=\linewidth]{../image_dump/Reconst_PCA_100}
%  %\caption{Rate 530 nats}\label{fig:awesome_image2}
%\endminipage\hfill
%\minipage{0.16\textwidth}
%  \includegraphics[width=\linewidth]{../image_dump/Reconst_PCA_500}
%  %\caption{Rate 1172 nats}\label{fig:awesome_image2}
%\endminipage\hfill
%\minipage{0.16\textwidth}
%  \includegraphics[width=\linewidth]{../image_dump/Original_Image}
%  %\caption{Original Image}\label{fig:awesome_image2}
%\endminipage\hfill
%\caption{PCA}
%\end{figure}
%
%\subsection{Classification Performance on MNIST}
%
%\begin{figure}[H]
%\centering
%\includegraphics{../image_dump/PBAvsPCA_MNIST}
%\caption{Classification Accuracy vs Rate comparison for PBA and PCA}
%\end{figure}



==> pba-tex 2/glodef.tex <==
% Theorem-like environments

\newtheorem{Theorem}{Theorem}
\newtheorem{Theorem*}{Theorem}

\newtheorem{Claim}[Theorem]{Claim}
\newtheorem{Claim*}[Theorem]{Claim}
\newtheorem{Corollary}[Theorem]{Corollary}
\newtheorem{Conjecture}[Theorem]{Conjecture}
\newtheorem{CounterExample*}{$\overline{\hbox{\bf Example}}$}
\newtheorem{Definition}[Theorem]{Definition}
\newtheorem{Example}[Theorem]{Example}
\newtheorem{Example*}[Theorem]{Example}
\newtheorem{Exercise}[Theorem]{Exercise}
\newtheorem{Intuition*}[Theorem]{Intuition}
\newtheorem{Joke*}[Theorem]{Joke}
\newtheorem{Lemma}[Theorem]{Lemma}
\newtheorem{Lemma*}[Theorem]{Lemma}
\newtheorem{Open problem}[Theorem]{Open problem}
\newtheorem{Proposition}[Theorem]{Proposition}
\newtheorem{Property}[Theorem]{Property}
\newtheorem{Question}[Theorem]{Question}
\newtheorem{Question*}[Theorem]{Question}
\newtheorem{Remark}[Theorem]{Remark}
\newtheorem{Result}[Theorem]{Result}
\newtheorem{Fact}[Theorem]{Fact}
\newtheorem{Condition}[Theorem]{Condition}

\usepackage{fullpage}

\newtheorem{theorem}{Theorem}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{example}[theorem]{Example}
\newtheorem{definition}[theorem]{Definition}


\newcommand{\prob}{{\rm Pr}}

% Begin / End Theorems

\def \bthm#1{\begin{#1}\upshape\quad}
\def \ethm#1{\rqed\end{#1}}
\def \ethmp#1{\end{#1}}     % No box, when ends in displayed equation

\def \bClaim     {\bthm{Claim}}
\def \eClaim     {\ethm{Claim}}
\def \eClaimp    {\ethmp{Claim}}
\def \bConjecture {\bthm{Conjecture}}
\def \eConjecture {\ethm{Conjecture}}
\def \eConjecturep{\ethmp{Conjecture}}
\def \bCorollary {\bthm{Corollary}}
\def \eCorollary {\ethm{Corollary}}
\def \eCorollaryp{\ethmp{Corollary}}
\def \bCounter   {\bthm{CounterExample*}}
\def \eCounter   {\ethm{CounterExample*}}
\def \eCounterp  {\ethmp{CounterExample}}
\def \bDefinition{\bthm{Definition}}
\def \eDefinition{\ethm{Definition}}
\def \eDefinitionp{\ethmp{Definition}}
\def \bExample   {\bthm{Example}}
\def \eExample   {\ethm{Example}}
\def \eExamplep  {\ethmp{Example}}
\def \bExercise  {\bthm{Exercise}}
\def \eExercise  {\ethm{Exercise}}
\def \eExercisep {\ethmp{Exercise}}
\def \bIntuition {\bthm{Intuition}}
\def \eIntuition {\ethmp{Intuition}}
\def \bJoke      {\bthm{Joke}}
\def \eJoke      {\ethm{Joke}}
\def \bLemma     {\bthm{Lemma}}
\def \eLemma     {\ethm{Lemma}}
\def \eLemmap    {\ethmp{Lemma}}
\def \bOpen      {\bthm{Open problem}}
\def \eOpen      {\ethm{Open problem}}
\def \eOpenp     {\ethmp{Open problem}}
\def \bProperty  {\bthm{Property}}
\def \eProperty  {\ethm{Property}}
\def \ePropertyp {\ethmp{Property}}
\def \bQuestion  {\bthm{Question}}
\def \eQuestion  {\ethm{Question}}
%\def \bRemark    {\bthm{Remark}}
%\def \eRemark    {\ethm{Remark}}
\def \bResult    {\bthm{Result}}
\def \eResult    {\ethm{Result}}
\def \bTheorem   {\bthm{Theorem}}
\def \eTheorem   {\ethm{Theorem}}
\def \eTheoremp  {\ethmp{Theorem}}

\def \bSubexa    {\begin{subexa}}
\def \eSubexa    {\ethm{subexa}}
\def \eSubexap   {\ethmp{subexa}}

% Environments

\usepackage[colorinlistoftodos,textsize=scriptsize]{todonotes}


\newenvironment{Problem}{\textbf{Problem}\\ \begin{enumerate}}{\end{enumerate}}
\newenvironment{Problems}{\textbf{Problems}\\ \begin{enumerate}}{\end{enumerate}}

%\newenvironment{Problems}{\begin{trivlist}\item[]{\textbf{Problems}}{\end{trivlist}}}

% Headers

\def \skpbld#1{\par\noindent\textbf{#1}\quad}
\def \skpblds#1{\skpbld{#1}\par\noindent}

\def \Answer   {\skpbld{Answer}}
\def \Answers  {\skpblds{Answers}}
\def \Basis    {\skpbld{Basis}}
\def \Check    {\skpbld{Check}}
%\def \Example  {\skpbld{Example}}
\def \Examples {\skpbld{Examples}}
\def \Intuition{\skpbld{Intuition}}
\def \Method   {\skpbld{Method}}
\def \Methods  {\skpblds{Methods}}
\def \Outline  {\skpbld{Outline}}
\def \Proof    {\skpbld{Proof}}
\def \Proofs   {\skpblds{Proofs}}
%\def \Problem  {\skpbld{Problem}}
%\def \Problems {\skpblds{Problems}}
\def \Proline  {\skpbld{Proof Outline}}
%\def \Remark   {\skpbld{Remark}}
\def \Remarks  {\skpblds{Remarks}}
\def \Solution {\skpbld{Solution}}
\def \Solutions{\skpblds{Solutions}}
\def \Verify   {\skpbld{Verify}}
\def \Step     {\skpbld{Step}}

% Ignores

\newcommand{\ignore}[1]{}

% Problems & solutions

\newcommand{\problem}[1]{#1}
\newcommand{\solution}[1]{{\\ \bf Solution}\quad #1}
%\newcommand{\solution}[1]{\mbox{}\\ \medskip\noindent{\bf Solution\medskip}#1}
%\newcommand{\solution}[1]{}

\newcommand{\source}[1]{(Taken from~\cite{#1})}
%\newcommand{\source}[1]{}

\newcommand{\modifiedfrom}[1]{(Modified from~\cite{#1})}
%\newcommand{\modifiedfrom}[1]{}

\newcommand{\takenfrom}[1]{(Taken from~\cite{#1})}
%\newcommand{\takenfrom}[1]{}

\newcommand{\reportedby}[1]{Reported by #1.}
%\newcommand{\reportedby}[1]{}

\newcommand{\hint}[1]{Hint: #1}
%\newcommand{\hint}[1]{}

\newcommand{\joke}[1]{\footnote{#1}}
\newcommand{\trivia}[1]{\footnote{#1}}

% Equation formatting

\newcommand{\spreqn}[1]{{\qquad\text{#1}\qquad}}

% Blackboard fonts
\newcommand{\II}{\mathbb{I}} % Added by Theertha on April 16th 2013.
\newcommand{\EE}{\mathbb{E}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\NN}{\mathbb{N}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\PP}{\mathbb{P}}

% Number sets

\newcommand{\complex}{\CC}
\newcommand{\integers}{\ZZ}
\newcommand{\naturals}{\NN}
\newcommand{\positives}{\PP}
\newcommand{\rationals}{\QQ}
\newcommand{\reals}{\RR}

\newcommand{\realsge}{{\reals_{\ge}}}
\newcommand{\realsp}{\reals^+}
\newcommand{\integersp}{\integers^+}
\newcommand{\integerss}[1]{\integers_{\ge{#1}}}

% boldface

\def \ba     {{\bf a}}
\def \bx     {{\bf x}}
\def \by     {{\bf y}}

\def \bA     {{\bf A}}
\def \bB     {{\bf B}}
\def \bC     {{\bf C}}
\def \bD     {{\bf D}}
\def \bF     {{\bf F}}
\def \bG     {{\bf G}}
\def \bL     {{\bf L}}
\def \bQ     {{\bf Q}}
\def \bR     {{\bf R}}
\def \bS     {{\bf S}}
\def \bT     {{\bf T}}
\def \bX     {{\bf X}}
\def \bY     {{\bf Y}}
\def \bZ     {{\bf Z}}

% caligraphics

\def \cA     {{\cal A}}
\def \cB     {{\cal B}}
\def \cC     {{\cal C}}
\def \cD     {{\cal D}}
\def \cE     {{\cal E}}
\def \cF     {{\cal F}}
\def \cG     {{\cal G}}
\def \cH     {{\cal H}}
\def \cI     {{\cal I}}
\def \cK     {{\cal K}}
\def \cL     {{\cal L}}
\def \cM     {{\cal M}}
\def \cN     {{\cal N}}
\def \cO     {{\cal O}}
\def \cP     {{\cal P}}
\def \cQ     {{\cal Q}}
\def \cR     {{\cal R}}
\def \cS     {{\cal S}}
\def \cT     {{\cal T}}
\def \cU     {{\cal U}}
\def \cV     {{\cal V}}
\def \cW     {{\cal W}}
\def \cX     {{\cal X}}
\def \cY     {{\cal Y}}
\def \cZ     {{\cal Z}}

% vectors

\def \vct#1{{\overline{#1}}}

\def \vcta  {{\vct a}}
\def \vctb  {{\vct b}}
\def \vctq  {{\vct q}}
\def \vcts  {{\vct s}}
\def \vctu  {{\vct u}}
\def \vctv  {{\vct v}}
\def \vctx  {{\vct x}}
\def \vcty  {{\vct y}}
\def \vctz  {{\vct z}}
\def \vctp  {{\vct p}}

\def \vctV  {{\vct V}}
\def \vctX  {{\vct X}}
\def \vctY  {{\vct Y}}
\def \vctZ  {{\vct Z}}

\def \vctbeta  {{\vct\beta}}

% Random variables

\newcommand{\rnd}[1]{{\boldsymbol #1}}

\newcommand{\rndd}{{\rnd d}}
\newcommand{\rndl}{{\rnd l}}
\newcommand{\rndp}{{\rnd p}}
\newcommand{\rnds}{{\rnd s}}
\newcommand{\rndx}{{\rnd x}}
\newcommand{\rndy}{{\rnd y}}
\newcommand{\rndz}{{\rnd z}}

%\newcommand{\poi}{{\rm poi}}
\newcommand{\Var}{{\rm Var}}

% following should not exist (indicate random sets)

\newcommand{\rndR}{{\rnd R}}
\newcommand{\rndT}{{\rnd T}}

% arrow vectors

\newcommand{\rvc}{{\overrightarrow c}}

% Abbreviations - \xspace puts space iff there is space after command

\newcommand{\eg}{\textit{e.g.,}\xspace}
\newcommand{\ie}{\textit{i.e.,}\xspace}  % note that overridden in spanish
%\newcommand{\iid}{\textit{i.i.d.}\xspace} 
\newcommand{\iid}{\textit{i.i.d.}} % Edit by Theertha, \xspace not compiling

\newcommand{\etc}{etc.\@\xspace}

% Colors

%\definecolor{light}{gray}{.75}


% marginal notes

\newcommand{\mrgs}[2]{\# #1 \#{\marginpar{#2}}}

\newcommand{\mrgcgd}[1]{\mrgs{#1}{CHANGED}}
\newcommand{\mrgchk}[1]{\mrgs{#1}{CHECK}}
\newcommand{\mrgfix}[1]{\mrgs{#1}{FIX}}
\newcommand{\mrgnew}[1]{\mrgs{#1}{NEW}}

% qed's --  Also consider \qedhere

\def \eqed    {\eqno{\qed}}
\def \rqed    {\hbox{}~\hfill~$\qed$}

% sequences

\def \upto  {{,}\ldots{,}}

\def \zn    {0\upto n}
\def \znmo  {0\upto n-1}
\def \znpo  {0\upto n+1}
\def \ztnmo {0\upto 2^n-1}
\def \ok    {1\upto k}
\def \on    {1\upto n}
\def \onmo  {1\upto n-1}
\def \onpo  {1\upto n+1}

% sets

\def \sets#1{{\{#1\}}}
\def \Sets#1{{\left\{#1\right\}}}

\def \set#1#2{{\sets{{#1}\upto{#2}}}}

\def \setpmo   {\sets{\pm 1}}
\def \setmpo   {\{-1{,}1\}}
\def \setzo    {\{0{,}1\}}
\def \setzn    {\{\zn\}}
\def \setznmo  {\{\znmo\}}
\def \setztnmo {\{\ztnmo\}}
\def \setok    {\{\ok\}}
\def \seton    {\{\on\}}
\def \setonmo  {\{\onmo\}}
\def \setzon   {\setzo^n}
\def \setzos   {\setzo^*}

\def \inseg#1{{[#1]}} % use \intsgm instead
\newcommand{\intsgm}[1]{{[#1]}}

% functions

\def \ord    {\#}

\def \suml   {\sum\limits}
\def \prodl  {\prod\limits}

% Set operations


%\DeclareMathOperator*{\union}{\cup}  %Commented by Theertha on April 15
%\DeclareMathOperator*{\Union}{\bigcup}  %Commented by Theertha on April 15

\newcommand{\unionl}{\union\limits}
\newcommand{\Unionl}{\Union\limits}
 
%\DeclareMathOperator*{\inter}{\cap}  %Commented by Theertha on April 15
%\DeclareMathOperator*{\Inter}{\bigcap}   %Commented by Theertha on April 15

\newcommand{\interl}{\inter\limits}
\newcommand{\Interl}{\Inter\limits}

% Floors, Ceilings, Absolute value

\def \ceil#1{{\lceil{#1}\rceil}}
\def \Ceil#1{{\left\lceil{#1}\right\rceil}}
\def \floor#1{{\lfloor{#1}\rfloor}}
\def \Floor#1{{\left\lfloor{#1}\right\rfloor}}
\def \absvlu#1{{|#1|}}
\def \Absvlu#1{{\left|{#1}\right|}}

% Parentheses, brackets

\def \paren#1{{({#1})}}
\def \Paren#1{{\left({#1}\right)}}
\def \brack#1{{[{#1}]}}
\def \Brack#1{{\left[{#1}\right]}}

%\def \frac#1#2{{{#1}\over{#2}}}
\def \frc#1#2{{\frac{#1}{#2}}}

\def \binomial#1#2{{{#1}\choose{#2}}}

\def \gcd#1#2{{{\rm gcd}\paren{{#1},{#2}}}}
\def \Gcd#1#2{{{\rm gcd}\Paren{{#1},{#2}}}}

\def \lcm#1#2{{{\rm lcm}\paren{{#1},{#2}}}}
\def \Lcm#1#2{{{\rm lcm}\Paren{{#1},{#2}}}}

% number theory

\newcommand{\base}[2]{{[#1]_{#2}}}

% equalities

\newcommand{\ed}{\stackrel{\mathrm{def}}{=}}

\newcommand{\cnvprb}{\stackrel{\mathrm{p}}{\to}}
\newcommand{\cnvdst}{\stackrel{\mathrm{d}}{\to}}
\newcommand{\cnvas}{\stackrel{\mathrm{a.s.}}{\to}}

\def \gap    {\ \hbox{\raisebox{-.6ex}{$\stackrel{\textstyle>}{\sim}$}}\ }

\newcommand{\al}[1]{\stackrel{\mathit{{#1}}}{<}}
\newcommand{\ag}[1]{\stackrel{\mathit{{#1}}}{>}}
\newcommand{\ale}[1]{\stackrel{\mathit{{#1}}}{\le}}
\newcommand{\age}[1]{\stackrel{\mathit{{#1}}}{\ge}}
\newcommand{\aeq}[1]{\stackrel{\mathit{{#1}}}{=}}

%\newcommand{\eae}{\approx} % exponentially asymptotically eq - replace by \ere
%\newcommand{\eal}{\stackrel<\approx} % replace by \erl

\newcommand{\re}{\sim}
\newcommand{\rle}{\stackrel<\sim} % roughly (asymptotically taken) <=
%\newcommand{\rl}{\stackrel<\sim}
\newcommand{\rge}{\stackrel>\sim}
%\newcommand{\rg}{\stackrel>\sim}

\newcommand{\ere}{\approx} % exponentially roughly equal
\newcommand{\erle}{\stackrel<\approx}
%\newcommand{\erl}{\stackrel<\approx}
\newcommand{\erge}{\stackrel>\approx}
%\newcommand{\erg}{\stackrel>\approx}

% Relations

\newcommand{\independent}{\perp\!\!\!\perp}

% values

\def \half    {{\frac12}}
\def \quarter {{\frac14}}
\def \oo#1{{\frac1{#1}}}

% notation

\def \iff    {{\it iff }}
\def \th     {{\rm th }}

% ignore

\def\ignore#1{}

% Logic

\newcommand{\ra}{\rightarrow}
\def \contra {{\leftrightarrows}}
\newcommand{\ol}[1]{{\overline{#1}}}
%\def \ob {\overline}

\def \ve {{\lor}} % needed?
\def \eq {{\equiv}} % needed?

% spaces

\newcommand{\spcin}{\hspace{1.0in}}
\newcommand{\spchin}{\hspace{.5in}}

% Default text appears in regular print in both book and class versions. 
% There are two types of text that need to be highlighted in class:
% clson - not mentioned in book version (eg jokes)
% clsbk - regular text in book (the parts that need be said)

%For book:
%\newcommand{\clson}[1]{}
%\newcommand{\clsbk}[1]{#1}
%For class:
\newcommand{\clson}[1]{\colorbox{light}{{#1}}}
\newcommand{\clsbk}[1]{\colorbox{light}{{#1}}}

%\newcommand{\bi}{\begin{aopl}}
%\newcommand{\ei}{\end{aopl}}

\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}
%\newcommand{\bq}{\begin{quote}}
%\newcommand{\eq}{\end{quote}}

\newenvironment{aopl}
  {\begin{list}{}{\setlength{\itemsep}{4pt plus 2pt minus 2pt}}}
  {\end{list}}

% operators

\newcommand{\flnpwr}[2]{{#1^{\underline{#2}}}} % Falling power

\def\orpro{\mathop{\mathchoice
   {\vee\kern-.49em\raise.7ex\hbox{$\cdot$}\kern.4em}
   {\vee\kern-.45em\raise.63ex\hbox{$\cdot$}\kern.2em}
   {\vee\kern-.4em\raise.3ex\hbox{$\cdot$}\kern.1em}
   {\vee\kern-.35em\raise2.2ex\hbox{$\cdot$}\kern.1em}}\limits}

\def\andpro{\mathop{\mathchoice
 {\wedge\kern-.46em\lower.69ex\hbox{$\cdot$}\kern.3em}
 {\wedge\kern-.46em\lower.58ex\hbox{$\cdot$}\kern.25em}
 {\wedge\kern-.38em\lower.5ex\hbox{$\cdot$}\kern.1em}
 {\wedge\kern-.3em\lower.5ex\hbox{$\cdot$}\kern.1em}}\limits}

\def\inter{\mathop{\mathchoice
   {\cap}
   {\cap}
   {\cap}
   {\cap}}}
\def\interl {\inter\limits}

\def\carpro{\mathop{\mathchoice
   {\times}
   {\times}
   {\times}
   {\times}}\limits}

\def\simge{\mathrel{%
   \rlap{\raise 0.511ex \hbox{$>$}}{\lower 0.511ex \hbox{$\sim$}}}}

\def\simle{\mathrel{
   \rlap{\raise 0.511ex \hbox{$<$}}{\lower 0.511ex \hbox{$\sim$}}}}

\newcommand{\pfx}{{\prec}}
\newcommand{\pfxeq}{{\preceq}}

\newcommand{\sfx}{{\succ}}
\newcommand{\sfxeq}{{\succeq}}

% for old documents

\newcommand{\twlrm}{\fontsize{12}{14pt}\normalfont\rmfamily}
\newcommand{\tenrm}{\fontsize{10}{12pt}\normalfont\rmfamily}

% picture macros

\newcommand{\grid}[2]{				% grid{width}{height}
  \multiput(0,0)(1,0){#1}{\line(0,1){#2}}
  \put(#1,0){\line(0,1){#2}}
  \multiput(0,0)(0,1){#2}{\line(1,0){#1}}
  \put(0,#2){\line(1,0){#1}}
}

%% \email{} command
\providecommand{\email}[1]{\href{mailto:#1}{\nolinkurl{#1}\xspace}}

%probabilities
\newcommand{\pr}{{p}} % phase out in favor of \prb
\newcommand{\prb}{{p}} 

\newcommand{\prbs}[1]{{\prb^{(#1)}}}

\newcommand{\Prb}{\text{Pr}}
%\newcommand{\Pr}{{\text{Pr}}} % phase out in favor of \Prb
\newcommand{\Prn}{\text{Pr}}  % phase out in favor of \Prb

\newcommand{\Prs}[1]{\Pr\Paren{#1}} % phase out in favor of \Prbs
\newcommand{\Prbs}[1]{{\Prb^{(#1)}}} % Check if used - phase out
\newcommand{\probof}[1]{\Pr\Paren{#1}}


% probability
\newcommand{\expectation}[1]{\EE\left[#1\right]}
\newcommand{\variance}[1]{Var\left(#1\right)}

%\newcommand{\qedsymbol}{\ensuremath{\blacksquare}}

%\newcommand{\qed}{\hfill\ensuremath{\blacksquare}}%


% inductiion macros

%\newcommand{\induction}[3]{
%Inductive statement: {#1}\\
%We prove: {#2}\\
%Basis: {#3}\\
%Step: {#4}\\
%Proof of step: {#5}
%}


==> pba-tex 2/intro.tex <==
\section{Introduction}

\emph{Autoencoders} are an effective method for representation learning
and dimensionality reduction. Given a centered dataset $\data_1, \data_2, \ldots, \data_n
\in \mathbb{R}^d$ (i.e., $\sum_i \data_i = 0$),
an autoencoder (with \emph{latent dimension} $k \le d$)
consists of an \emph{encoder} $f:
\mathbb{R}^d \mapsto \mathbb{R}^k$ and a \emph{decoder} $g: \mathbb{R}^k \mapsto
\mathbb{R}^d$. The goal is to select $f$ and $g$ from prespecified
classes $\mathcal{C}_f$ and $\mathcal{C}_g$ respectively such that if a random point $\data$ is picked from the data set then $g(f(\data))$ is close to $\data$ in some sense, for example in mean squared error. 
If $\mathcal{C}_f$ and $\mathcal{C}_g$ consist of linear mappings then the autoencoder is called a \emph{linear autoencoder}.

Autoencoders have achieved striking successes when $f$ and $g$ are
selected through training from the class of functions realized
by multilayer perceptrons of a given architecture~\cite{HintonS06}.
Yet, the canonical autoencoder formulation described above has
a notable failing, namely that for linear autoencoders,
optimal choices of $f$ and $g$ do not necessarily identify the 
principal components of the dataset; they merely identify the principal
subspace~\cite{BourlardK88, BaldiH89}. That is, the components of $f(\data)$ 
are not necessarily proportional to projections of $\data$ against the eigenvectors of the covariance matrix
\begin{equation}\label{eq:cov}
\cov\ed \frac{1}{n} \sum_{i = 1}^n \data_i \cdot \data_i^\top,
\end{equation}
which we assume without loss of generality is full rank.
Thus, linear autoencoders do not recover Principal Component
Analysis (PCA). The reason {for this} is that both the objective 
(the distortion) and the constraint (the dimensionality
of the latents) are invariant to an invertible transformation 
applied after the encoder with its inverse applied 
before the decoder. It is desirable for linear autoencoders to recover PCA for two reasons. First, from a representation learning standpoint, it guarantees that the autoencoder recovers uncorrelated features. Second, since a conventional linear autoencoder has a large number of globally optimal solutions corresponding to different bases of the principal subspace, it is preferable to eliminate this indeterminism.

Autoencoders are sometimes described as ``compressing'' the
data~\cite{Santo12,BourlardK88, LiaoZWLL21, Bishop06}, even though $f$
can be invertible even when $k < d$.
We show that by embracing this {compression-}view, one can obtain 
autoencoders that are {able} to recover PCA.
%The second limitation is that the problem is degenerate in
%the sense that there exist invertible maps from $\mathbb{R}^d$ to $[0,1]$ 
%for any $d \ge 1$. While one can avoid such degenerate solutions
%by constraining the class $\mathcal{C}_f$, this inevitably
%limits the ability of the autoencoder to disentangle complex
%dependencies within the data.
%In this paper, we embrace this view and
%show that formulating the autoencoder problem in terms of 
%compression, rather than dimensionality reduction, 
%addresses both issues. 
%%Although the resulting
%solutions do not reduce the dimensionality of the data to
%the same extent, we shall see that they still reduce it
%considerably while affording other benefits.
%Classical rate-distortion theory \cite{CoverT06} requires that the compressed
%representation be discrete, and it measures the amount of compression
%through the size of its range (or its entropy). This allows
%for arbitrarily complex encoders and decoders
%while still avoiding the degeneracy noted above.  
Specifically, we consider linear autoencoders with quantized (or,
equivalently, noisy) latent variables with a constraint on the estimated
number of bits required to transmit the quantized latents
under fixed-rate coding. We call this problem 
\emph{Principal Bit Analysis (PBA).}
% TODO: is PBA the problem or the solution?
The constraint turns out to be a strictly Schur-concave
function of the set of variances of the latent variables (see 
the supplementary for a review of Schur-concavity). Although
finding the optimal $f$ and $g$ for this loss function is
a nonconvex optimization problem,  we
show that for any strictly Schur-concave loss function,
an optimal $f$ must send projections of the data along the 
principal components, assuming that the empirical covariance
matrix of the data has only simple eigenvalues. That is,
imposing a strictly Schur-concave loss in place of a
simple dimensionality constraint suffices to ensure recovery of PCA.
The idea is that the strict concavity of the loss function 
eliminates the rotational invariance described above.
As we show, even a slight amount of ``curvature'' in the 
constraint forces the autoencoder to spread the variances
of the latents out as much as possible, resulting in recovery
of PCA. If the loss function is merely Schur-concave, then 
projecting along the principal components is optimal, but 
not necessarily uniquely so. 

Using this theorem, we can efficiently solve PBA.
We validate the solution experimentally by using it to construct
a fixed-rate compression algorithm for arbitrary vector-valued
data sources.  We find that the PBA-derived compressor  beats
existing linear, fixed-rate compressors both in terms of
mean squared error, for which it is optimized, and in terms
of the structural similarity index measure (SSIM) and downstream
classification accuracy, for which it is not. 

A number of variable-rate multimedia compressors have recently
been proposed that are either related to, or directly
inspired by, autoencoders \cite{TschannenAL18, TodericiVJHMSC17,
BalleLS16, TodericiOHVMBCS16, TheisSCH17, RippelB17, HabibianRTC19,
AgustssonMTCTBG17, BalleMSHJ18, ZhouCGSW18, AgustssonTMTG19, BalleCMSJAHT20}. 
As a second application of our result,
we show that for Gaussian sources, a linear form of such a
compressor is guaranteed to recover PCA. Thus we show that
ideas from compression can be fruitfully fed back into the
original autoencoder problem.

The contributions of the paper are
\begin{itemize}
\item We propose a novel linear autoencoder formulation in which
	the constraint is Schur-concave. We show that this generalizes
      conventional linear autoencoding.
\item If the constraint is strictly Schur-concave and the 
        covariance matrix of the data has only simple 
       eigenvalues, then we show that the autoencoder
       provably recovers PCA, providing a new remedy
       for a known limitation of linear autoencoders.
\item We use the new linear autoencoder formulation to efficiently
	  solve a fixed-rate compression problem that we
       call \emph{Principal Bit Analysis (PBA).}
\item We demonstate experimentally that PBA outperforms
	 existing fixed-rate compressors on a variety
		of data sets and metrics.
\item We show that a linear, variable-rate compressor that 
      is representative of many autoencoder-based
	compressors in the literature effectively has
       a strictly Schur-concave loss, and therefore it
		recovers PCA.
\end{itemize}

%Most recent successes of autoencoder-based compression have been in the realm of variable-rate compression wherein a rate-distortion Lagrangian is optimized via gradient-based optimization methods to yield a compressor \cite{TschannenAL18}, \cite{TodericiVJHMSC17}, \cite{BalleLS16}, \cite{TodericiOHVMBCS16}, \cite{TheisSCH17}, \cite{RippelB17}, \cite{HabibianRTC19}. However, these have been less understood theoretically. As a first step towards characterizing the performance of variable-rate autoencoder-based compressors, we consider their performance on the theoretically well-studied Gaussian sources. Although the PBA formulation is obtained via fixed-rate compression, we use it to show that a linear autoencoder suffices to achieve the optimal rate of reconstructing a zero-mean Gaussian source within 0.255 bits per dimension.
%TODO: this only holds for mean-square error.

%We also consider a generalization of PBA 
%that penalizes both the number of bits needed to represent the 
%latent variables as well as their dimensionality, which we solve 
%explicitly. We show this recovers PBA and PCA as special cases, 
%providing a new algorithm that simultaneously generalizes PCA and 
%reverse waterfilling, placing the two on a common footing.

% TODO: point out that if non-strictly Schur concave, then out
% result cannot be improved in that we might only recover the
% subspaces.

% TODO: the Schur concave part is only part of the loss funcion



==> pba-tex 2/locdef.tex <==

\newcommand{\Xon}{X^\ns}

%\usepackage[document]{ragged2e}

%\topmargin0.0cm
%\headheight0.0cm
%\headsep0.0cm
%\oddsidemargin0.0cm
%\textheight23.0cm
%\textwidth16.5cm
%\footskip1.0cm
%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{corollary}{Corollary}
%\newtheorem{lemma}{Lemma}
%\newtheorem{proposition}{Proposition}
%\newtheorem{conjecture}{Conjecture} 
%\newtheorem{question}{Question} 
%\theoremstyle{definition}
%\newtheorem{definition}{Definition}[section]




\def\fulldetails{0}

\ifnum\withcolors=1
  \newcommand{\new}[1]{{\color{red} {#1}}} % new
  \newcommand{\newer}[1]{{\color{blue} {#1}}} % even newer
  \newcommand{\newest}[1]{{\color{orange} {#1}}} % even even newer
  \newcommand{\newerest}[1]{{\color{blue!10!black!40!green} {#1}}} % you get the idea.
  \newcommand{\acolor}[1]{{\color{purple}#1}} % Jayadev
  \newcommand{\bcolor}[1]{{\color{cyan}#1}} % Sourbh
  \newcommand{\wcolor}[1]{{\color{orange}#1}} % Aaron
  
\else
  \newcommand{\new}[1]{{{#1}}}
  \newcommand{\newer}[1]{{{#1}}}
  \newcommand{\newest}[1]{{{#1}}}
  \newcommand{\newerest}[1]{{{#1}}}
  \newcommand{\acolor}[1]{{#1}}
  \newcommand{\bcolor}[1]{{#1}}
\fi

\ifnum\withnotes=1
  \newcommand{\anote}[1]{\par\acolor{\textbf{JA: }\sf #1}} % 
  \newcommand{\bnote}[1]{\par\bcolor{\textbf{SB: }\sf #1}} % 
  \newcommand{\wnote}[1]{\par\scolor{\textbf{AW: }\sf #1}} % 
  \newcommand{\afootnote}[1]{\footnote{{\bf \acolor{Jayadev}}: {#1}}}


  \newcommand{\todonote}[2][]{\todo[size=\scriptsize,color=red!40,#1]{#2}}  
	\newcommand{\questionnote}[2][]{\todo[size=\tiny,color=blue!30]{#2}}
	\newcommand{\todonotedone}[2][]{\todo[size=\scriptsize,color=green!40]{$\checkmark$ #2}}
	\newcommand{\todonoteinline}[2][]{\todo[inline,size=\scriptsize,color=orange!40,#1]{#2}}  
  \newcommand{\marginnote}[1]{\todo[color=white,linecolor=black]{{#1}}}
\else
  \newcommand{\anote}[1]{}
  \newcommand{\bnote}[1]{}
  \newcommand{\wnote}[1]{}
  \newcommand{\todonote}[2][]{\ignore{#2}}
	\newcommand{\questionnote}[2][]{\ignore{#2}}
	\newcommand{\todonotedone}[2][]{\ignore{#2}}
	\newcommand{\todonoteinline}[2][]{\ignore{#2}}
  \newcommand{\marginnote}[1]{\ignore{#1}}
\fi
\newcommand{\amargin}[1]{\questionnote{\acolor{#1}}} % Jayadev
\newcommand{\bmargin}[1]{\questionnote{\bcolor{#1}}} % Sourbh
\newcommand{\wmargin}[1]{\questionnote{\scolor{#1}}} % Aaron

\newcommand{\eps}{\varepsilon}
%VAE Macros 
\newcommand{\trp}{p_{\text{data}}}
\newcommand{\pcnd}[3][]{
\ifthenelse{\equal{#1}{}}{p\left(#2 \middle| #3\right)}{p_{#1} \left(#2 \middle| #3 \right)}
}
\newcommand{\qcnd}[3][]{
\ifthenelse{\equal{#1}{}}{q\left(#2 \middle| #3\right)}{q_{#1} \left(#2 \middle| #3 \right)}
}
\newcommand{\qjnt}[3][]{
\ifthenelse{\equal{#1}{}}{q\left(#2, #3\right)}{q_{#1} \left(#2 , #3 \right)}
}
\newcommand{\pjnt}[3][]{
\ifthenelse{\equal{#1}{}}{p\left(#2, #3\right)}{p_{#1} \left(#2,#3 \right)}
}
\newcommand{\qmrg}[2][]{
\ifthenelse{\equal{#1}{}}{q\left(#2 \right)}{q_{#1} \left(#2 \right)}
}
\newcommand{\pmrg}[2][]{
\ifthenelse{\equal{#1}{}}{p\left(#2 \right)}{p_{#1} \left(#2 \right)}
}

\DeclarePairedDelimiterX{\infdivx}[2]{(}{)}{%
  #1\|#2%
}
%\newcommand{\kl}[2]{ D_{\text{KL}}\left(#1 \lvert \rvert #2\right)}
\newcommand{\infdiv}{D_{KL}\infdivx}
\newcommand{\elbo}{\cL\left(\lambda,\theta,x\right)}

\newcommand{\expc}[2][]{\ifthenelse{\equal{#1}{}} {\mathbb{E}\left[ #2 \right] }{\mathbb{E}_{#1} \left[ #2 \right]}}
\newcommand{\qcndlam}{q_{\lambda}\left( z \middle| x \right)}
\newcommand{\pcndthe}{p_{\theta}\left( x \middle| z \right)}
\newcommand{\pdata}{p_{\text{data}}(x)}
\newcommand{\ipdim}{d}
\newcommand{\ldim}{r}
\newcommand{\encmat}{W_{\lambda}}
\newcommand{\decmat}{T_{\theta}}
\newcommand{\encmeanmat}{U_{\lambda}}
\newcommand{\encvarmat}{V_{\lambda}}
\newcommand{\diag}{\text{diag}}
\DeclareMathOperator*{\E}{\mathbb{E}}
\newcommand{\tr}{\text{tr}}
\newcommand{\cov}{\bm{K}}
\newcommand{\dcov}{\bm{\Lambda}}
\newcommand{\encnew}{\bm{W}}
\newcommand{\encvec}{\bm{w}}
\newcommand{\decnew}{\bm{T}}
\newcommand{\lagmlt}{\nu}
\newcommand{\ort}{\bm{Q}}
\newcommand{\ortvec}{\bm{q}}
\newcommand{\ide}{\bm{I}}
\newcommand{\encv}[2][]{\ifthenelse{\isempty{#1}}{\bm{w}_{#2}}{w_{#1 #2}}}
\newcommand{\sigpr}{\sigma_1'}
\newcommand{\rotencv}[2][]{\ifthenelse{\isempty{#1}}{\bm{y}_{#2}}{y_{#1 #2}}}
\newcommand{\cdir}{b} % coupled direction
%\newcommand{\argmin}{\text{argmin}}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\newcommand{\mdiag}{\tilde{d}} %eigenvalues of modified matrix
\newcommand{\eigv}{v}
\newcommand{\eigmin}[1]{\tilde{d}_{\text{min},#1}}
%\newcommand{\encvec}[1]{\bm{W}_{#1}}
\newcommand{\deltaW}{\bm{Z}}
\newcommand{\diffW}{\delta \bm{W}}
%\newcommand{\sq_norm}[1]{\left \lVert #1 \right \rVert_2}

%Fresh Macros for PBA
\newcommand{\data}{\bm{x}}
\newcommand{\latent}{\bm{y}}
\newcommand{\code}{\bm{z}}
\newcommand{\scale}{\beta}
\newcommand{\diagcov}{\bm{\Sigma}}
\newcommand{\lb}{L}
\newcommand{\distortion}{D}
\newcommand{\scalePBA}{\alpha}
\newcommand{\fenc}{f}
\newcommand{\fdec}{g}
\newcommand{\noise}{\bm{\eps}}
\newcommand{\noisevar}{\sigma^2}
\newcommand{\rateproxy}{\rho}
\newcommand{\eigvec}{\bm{u}}
\newcommand{\eigmat}{\bm{U}}
\newcommand{\diagenc}{\widetilde{\bm{W}}}
\newcommand{\var}{\bm{y}}
\newcommand{\setY}{\cY}
\newcommand{\setW}{\cW}
\newcommand{\vort}{\bm{Y}}
\newcommand{\vortvec}{\bm{p}}
\newcommand{\sendopt}{r^*}
\newcommand{\send}{r}
\newcommand{\sendmax}{r_{\text{max}}}
\newcommand{\GM}{\text{GM}}
\newcommand{\sendoptimal}{r_{\text{opt}}}
\newcommand{\num}{n}
\newcommand{\encunit}{\bm{V}}
\newcommand{\encunitvec}{\bm{v}}
\newcommand{\scaling}{s}
\newcommand{\scalemat}{\bm{S}}
\newcommand{\decunit}{\bm{V}_d}
\newcommand{\genmat}{\bm{M}}
\newcommand{\genmatvec}{\bm{m}}
\newcommand{\genvec}{\bm{v}}
\newcommand{\lag}{\cL}
\newcommand{\setD}{\left \lbrace D_i \right \rbrace_{i=1}^{d}}
\newcommand{\setmu}{\left \lbrace \mu_i  \right \rbrace_{i=1}^{d}}
\newcommand{\orthvar}{\mu}


==> pba-tex 2/opti.tex <==
%\section{Notation}
%We denote matrices by bold capital letters e.g. $\genmat$, and vectors by bold small, e.g. $\genvec$. The $j^{\text{th}}$ column of a matrix $\genmat$ is denoted by $\genmatvec_j$. We denote the $j^{\text{th}}$ entry of a vector $\genvec$ by $\left[\genvec\right]_j$. We denote the set $\left \lbrace 1, \cdots \ipdim \right \rbrace$ by $\left[ \ipdim \right]$ and the set of all binary strings of any lengnth (including the empty string) by $\{0,1\}^*$. A sequence $a_1, a_2, \cdots a_n$ is denoted by $\{a_i\}_{i=1}^{n}$. We denote the zero column by $\bm{0}$. Logs without bases are natural logarithms.

%Let $J \subseteq \left[ \ipdim \right] $ be an index set and let $C = \left \lbrace c_1 
%\cdots c_{\ipdim}\right \rbrace$  be a set then we denote $C_J = \left \lbrace c_j : j \in J \right \rbrace$. We assume all logs are to the base $2$ unless otherwise specified. 

\section{Linear Autoencoding with a Schur-Concave Constraint}\label{sec:FRAMEWORK}

Throughout this paper we consider $\mathcal{C}_f$ and 
$\mathcal{C}_g$ to be the class of linear functions. The 
functions $f\in\mathcal{C}_f$ and $g \in\mathcal{C}_g$ can then be represented by $d$-by-$d$ matrices, 
respectively, which we denote by
$\encnew$ and $\decnew$, respectively. Thus we have
\begin{align}
    f(\data) & = \encnew^\top \data \\
    g(\data) & = \decnew \data.
\end{align}
We wish to design $\encnew$ and $\decnew$ to
minimize the mean squared error when the latent variables
$\encnew^\top \data$ are quantized, subject to a constraint
on the number of bits needed to represent the quantized latents.
We accomplish this via two modifications of the canonical autoencoder.
First, we perturb the $d$ latent variables with zero-mean
additive noise with covariance matrix $\noisevar \ide$, which we denote by
$\noise.$ Thus the input to the decoder is 
\begin{equation}
\encnew^\top \data + \noise
\end{equation}
and our objective is to minimize the mean squared error
\begin{equation}
    \label{eq:1stmse}
 \frac{1}{n} \sum\limits_{i=1}^{n} \EE_{\noise}\left[ \left \lVert \data_i - \decnew\left( \encnew^\top\data_i+ \noise \right) \right \rVert_2^2 \right].
\end{equation}

This is equivalent to quantizing the latents, in the following sense~\cite{ZamirF92}.
Let $Q(\cdot)$ be the function that maps any real number to its nearest 
integer and $\eps$ be a random variable uniformly distributed over $[-1/2,1/2]$. Then for $X$ independent of $\eps$, the quantities $Q(X + \eps) - \eps$
and $X + \eps$ have the same joint distribution with $X$.
%TODO: what is our notation for random vs. deterministic?
% TODO: double-check statement of ditered quantization equivalence.
Thus (\ref{eq:1stmse}) is exactly the mean squared error if the latents
are quantized to the nearest integer and $\noisevar = \frac{1}{12}$, 
% TODO: double check variance of uniform
assuming that the quantization is dithered. The overall system is depicted
in Fig.~\ref{fig:blockdiag}.

% TODO: need to introduce generic $\rho function
%
%\begin{figure}[!htb]
%    \begin{center}
%  \includegraphics[width=\linewidth]{images/blockdiag.png}
%    \end{center}
%  %\caption{MNIST}\label{fig:mnist_mse}


\tikzstyle{block} = [rectangle, draw, text width=5em, text centered, rounded corners, minimum height=4em]
\tikzstyle{line} = [draw, -latex']
\tikzstyle{input} = [coordinate]
\begin{figure}[!htb]
\begin{center}
\begin{tikzpicture}[node distance=1cm, auto]
	\node [input, name=input] {};
    \node [block,right = 1.5cm of input] (A) {Linear Encoder ($\encnew$)};
    \node [block, right=1.5cm of A] (B) {Quantizer};
    \node [block, right=2cm of B] (C) {Linear Decoder ($\decnew$)};
    \node [text width = 1.5cm, right = 0.5cm of C] (D) {$\decnew\left(\encnew^\top \data_i + \bm{\eps} \right)$};
	\draw [draw,->] (input) -- node {$\data_i$} (A);
    \path [line] (A) -- node [text width=2cm,midway,above,align=center ] {$\encnew^\top \data_i$} (B);
    \path [line] (B) -- node [text width=2cm,midway,above,align=center ] {$\encnew^\top \data_i + \bm{\eps}$} (C);
    \path [line] (C) -- (D);

\end{tikzpicture}
\end{center}
\caption{Compression Block Diagram}\label{fig:blockdiag}
\end{figure}
We wish to constrain the number of bits needed to describe
the latent variables. We assume that the $j$th quantized latent
is clipped to the interval 
$$\left(-\frac{\sqrt{ (2a)^2 \encvec_j^\top \cov \encvec_j + 1}}{2},
\frac{\sqrt{(2a)^2 \encvec_j^\top \cov \encvec_j + 1}}{2}\right],$$ where
$a > 0$ is a hyperparameter and the covariance matrix $\cov$ is as defined in \eqref{eq:cov}. The idea is that for sufficiently
large $a$, the interval $$\left(-a\sqrt{ \encvec_j^\top \cov 
\encvec_j}, a\sqrt{ \encvec_j^\top \cov \encvec_j}\right]$$ 
contains the latent with high probability, and adding $1$
accounts for the expansion due to the dither. The number of
bits needed for the $j$th latent is then
\begin{align}
    \log \left(\sqrt{ 4a^2 \encvec_j^\top \cov \encvec_j + 1}\right)
      = \frac{1}{2} \log \left(4a^2 \encvec_j^\top \cov \encvec_j + 1\right).
\end{align}
We arrive at our optimization problem:
\begin{equation}\label{eq:MASTEROPTIPBA}
\begin{aligned}
\inf\limits_{\encnew,\decnew}  \quad & \frac{1}{n} \sum\limits_{i=1}^{n} \EE_{\noise}\left[ \left \lVert \data_i - \decnew\left( \encnew^\top\data_i+ \noise \right) \right \rVert_2^2 \right] \\ 
    \text{subject to} \quad & R \geq \sum_{j = 1}^d \frac{1}{2} \log \left(4a^2 \encvec_i^\top \cov \encvec_i + 1\right).
\end{aligned}
\end{equation}
% TODO: cf variable-rate compression
Note that the function 
$$\{\encvec_j^\top \cov \encvec_j\}_{j = 1}^d \mapsto \sum_{j = 1}^d \frac{1}{2} \log \left(4a^2 \encvec_i^\top \cov \encvec_i + 1\right)$$
is strictly Schur-concave (see Appendix~\ref{app:schur} for a brief review
of Schur-concavity). Our first result only requires that the constraint
is Schur-concave in the set of latent variances, so we will consider
the more general problem

\begin{equation}\label{eq:MASTEROPTI}
\begin{aligned}
\inf\limits_{\encnew,\decnew}  \quad & \frac{1}{n} \sum\limits_{i=1}^{n} \EE_{\noise}\left[ \left \lVert \data_i - \decnew\left( \encnew^\top\data_i+ \noise \right) \right \rVert_2^2 \right] \\ 
    \text{subject to} \quad & R \geq \rho\left(\left\{\encvec_j^\top \cov \encvec_j\right\}_{j = 1}^d\right)
\end{aligned}
\end{equation}
where $\rateproxy(\cdot)$ is any Schur-concave function.

Expressing the objective in~\eqref{eq:MASTEROPTI} in terms of $\cov$, the optimization problem reduces to
\begin{equation}\label{eq:MASTEROPTI_LIN}
\begin{aligned}
\inf \limits_{\encnew, \decnew}  \quad & \tr\left( \cov \right) - 2\tr\left(\cov \encnew \decnew^\top \right) + \tr\left( \decnew\left( \encnew^\top \cov \encnew + \noisevar\bm{I} \right) \decnew^\top \right) \\ 
\text{subject to} \quad & R \geq \rho\left(\left\{\encvec_j^\top \cov \encvec_j\right\}_{j = 1}^d\right).
\end{aligned}
\end{equation}

Since $\decnew$ does not appear in the rate constraint, the optimal $\decnew$ can be viewed as the Linear Least Squares Estimate (LLSE) of a random $\data$ given $\encnew^\top \data + \noise$. Therefore, the optimal decoder, $\decnew^*$ for a given encoder $\encnew$ is (e.g. \cite{Kay98}):

\begin{equation}
\decnew^* = \cov \encnew (\encnew^{\top} \cov \encnew + \noisevar\bm{I})^{-1}.
\end{equation}
Substituting for $\decnew$ in \eqref{eq:MASTEROPTI_LIN} yields an optimization problem over only $\encnew$
\begin{equation} \label{eq:MASTEROPTI_MMSE}
\begin{aligned} 
\inf\limits_{\encnew} \quad & \tr(\cov) - \tr(\cov \encnew (\encnew^{\top} \cov \encnew + \noisevar\bm{I} )^{-1}\encnew^{\top} \cov ) \\
\text{subject to} \quad & R \geq \rho\left(\left\{\encvec_j^\top \cov \encvec_j\right\}_{j = 1}^d\right).
\end{aligned}
\end{equation}

This problem is nonconvex in general.
In the following subsection, we prove a structural result about
the problem for a Schur-concave $\rateproxy$. Namely, we show that
the nonzero rows of $\encnew$ must be eigenvectors of $\cov$.
In Section~\ref{sec:PBAPCA}, we solve the problem for the specific 
choice of $\rateproxy$ in (\ref{eq:MASTEROPTIPBA}). We also show how this
generalizes conventional linear autoencoders.

\subsection{Optimal Autoencoding with a Schur-Concave Constraint}\label{subsec:PROOF}

%We now show that for a strictly Schur-concave $\rateproxy$, the optimal $\encnew$ for the optimization problem \eqref{eq:MASTEROPTI_MMSE} has all its columns aligned along the eigenvectors of $\cov$.

The following is the main theoretical result of the paper.

%\begin{theorem}\label{thm:diagisoptimal}
%Let $\cov$ be a covariance matrix with eigenvalues $\sigma_i^2$, $1\leq i \leq d$ such that $\sigma_1^2 \geq \sigma_2^2 \cdots \geq \sigma^2_d$. For a concave $\rateproxy:\RR_0^{+} \rightarrow \RR_0^{+}, R>0$ the optimal encoder $\encnew^*$ of \eqref{eq:MASTEROPTI_MMSE} is of the form $\eigvec \diagenc^*$ where $\eigvec$ is the matrix formed from the eigenvectors of $\cov$ and $\diagenc^*$ is a diagonal matrix. 
%\end{theorem}

%\begin{theorem}\label{thm:diagisoptimal}
%For a concave, nondecreasing $\rateproxy:\RR_0^{+} \rightarrow \RR_0^{+}, R>0$ any optimal encoder $\encnew^*$ of \eqref{eq:MASTEROPTI_MMSE} is of the form $\eigmat \diagenc^*$ where $\eigmat$ is the matrix whose columns are the eigenvectors of $\cov$ and $\diagenc^*$ is a diagonal matrix. 
%\end{theorem}

\begin{theorem}\label{thm:diagisoptimal}
For Schur-concave $\rateproxy:\RR_{\geq 0}^{d} \rightarrow \RR_{\geq 0}$ and $R>0$, the set of matrices whose nonzero columns are eigenvectors of the covariance matrix $\cov$ is optimal for \eqref{eq:MASTEROPTI_MMSE}. If $\rateproxy$ is strictly Schur-concave and $\cov$ contains distinct eigenvalues, this set contains all optimal solutions of \eqref{eq:MASTEROPTI_MMSE}.
\end{theorem}

\begin{proof}
%We first make a change of basis that allows us to restrict our attention to diagonal covariance matrices $\cov$. Consider the optimization problem 
%\begin{equation} \label{eq:MASTEROPTI_DIAG}
%\begin{aligned} 
%\min\limits_{\widetilde{\encnew}} \quad & \tr(\diagcov) - \tr(\diagcov\widetilde{\encnew} (\widetilde{\encnew}^{\intercal} \diagcov \widetilde{\encnew} + I )^{-1}\widetilde{\encnew}^{\intercal} \diagcov ) \\
%\text{s.t.} \quad & R \geq \sum\limits_{j=1}^{d} \rateproxy( \widetilde{\encnew}_j^{\intercal} \diagcov  \widetilde{\encnew}_j ).
%\end{aligned}
%\end{equation}
%where $\widetilde{\encnew} \in \RR^{\ipdim \times \ipdim}$ and $\diagcov$ is such that $\cov = \bm{U} \bm{\diagcov} \bm{U}^{\intercal}$ where $\diagcov$ is the diagonal matrix with eigenvalues on its diagonal of $\cov$. Substituting $\encnew = \bm{U} \widetilde{\encnew}$ in \eqref{eq:MASTEROPTI_MMSE} where $\widetilde{\encnew} \in \RR^{\ipdim \times \ipdim}$ gives \eqref{eq:MASTEROPTI_DIAG}. Since this is an invertible transformation, every solution of \eqref{eq:MASTEROPTI_DIAG} corresponds to a solution of \eqref{eq:MASTEROPTI_MMSE} implying that to solve \eqref{eq:MASTEROPTI_MMSE} we can equivalently analyze \eqref{eq:MASTEROPTI_DIAG} for a diagonal covariance matrices $\cov$. 

%It now remains to prove that the optimal $\diagenc^*$ of \eqref{eq:MASTEROPTI_DIAG} is a diagonal matrix. As a stepping stone, we prove that $\diagenc^{*T} \cov \diagenc^*$ is diagonal for a diagonal $\cov$. 


Let the eigenvalues of $\cov$ be $\{\sigma_i^2\}_{i=1}^{d}$ with $\sigma_1^2 \ge \sigma_2^2 \ge \ldots \ge \sigma^2_d$. Let the eigendecomposition of $\cov$ be given by $\cov = \eigmat \diagcov \eigmat^{\top}$ where $\eigmat$ is an orthogonal matrix whose columns are the eigenvectors of $\cov$ and $\diagcov$ is a diagonal matrix with entries $\left \lbrace \sigma_i^2 \right \rbrace_{i=1}^{d}$.

We first prove that the optimal value of \eqref{eq:MASTEROPTI_MMSE} can be achieved by \newest{a} $\encnew$ such that $\encnew^{\top} \cov \encnew$ is a diagonal matrix. Let $\diagenc = \encnew \ort$ where $\ort$ is the orthogonal matrix obtained from the eigendecomposition of $\encnew^{\top} \cov \encnew$ i.e., $$\encnew^{\top}\cov \encnew = \ort\dcov \ort^{\top},$$ where $\dcov$ is a diagonal matrix formed from the eigenvalues of $ \encnew^{\top}\cov \encnew$. Note that 
\begin{align*}
\tr \left( \cov \widetilde{\encnew} \left( \widetilde{\encnew}^{\top} \cov \widetilde{\encnew} + \noisevar\ide \right)^{-1} \widetilde{\encnew}^{\top} \cov\right) &= \tr \left( \cov \encnew \ort \left(  \dcov + \noisevar\ide \right)^{-1} \ort^{\top} \encnew^{\top} \cov \right) \\
&= \tr \left(  \cov \encnew \left( \ort \dcov \ort^{\top} + \noisevar\ort \ort^{\top} \right)^{-1} \encnew^{\top} \cov \right).
\end{align*}
Since $\ort \dcov \ort^{\top} = \encnew^{\top} \cov \encnew$ and $\ort \ort^{\top}= \ide$, the objective remains the same. 
We now show that the constraint is only improved. Denoting the eigenvalues of $\encnew^{\top} \cov \encnew$ by $\left \lbrace \nu_j \right \rbrace_{j=1}^d$, we have
\begin{equation*}
\rateproxy\left( \left \lbrace \widetilde{\encvec}_j^{\top} \cov \widetilde{\encvec}_j \right \rbrace_{j=1}^{\ipdim} \right) 
=  \rateproxy\left( \left \lbrace \ortvec_j^{\top} \encnew^{\top} \cov \encnew \ortvec_j \right \rbrace_{j=1}^{\ipdim} \right) =  \rateproxy \left( \left \lbrace  \nu_j \right \rbrace_{j=1}^{\ipdim} \right).
\end{equation*}
%    We know that the sum of eigenvalues of a matrix equals its trace, 
%    
%    \[\sum\limits_{j=1}^d \nu_j = \tr\left( \encnew^{\top} \cov \encnew \right) = \sum\limits_{j=1}^{d} \encvec_j^{\top} \cov \encvec_j. \] 
    
Now since the eigenvalues of a Hermitian matrix majorize its diagonal elements by the Schur-Horn theorem \cite[Theorem~4.3.45]{HornJ85},
$$ \left \lbrace \encvec_j^{\top} \cov \encvec_j \right \rbrace_{j=1}^{d} \prec \left \lbrace \nu_j \right \rbrace_{j=1}^{\ipdim}.$$
%Define $h:\RR^d \rightarrow \RR$ where $h\left(b\right) =  \sum\limits_{j=1}^{d} \rateproxy \left( b_j\right) $. Since $h$ is a sum of concave functions, it is concave. It is also symmetric in the coordinates and therefore Schur concave. 
Since $\rateproxy$ is Schur-concave, this implies
%$$ \sum\limits_{j=1}^{d} \rateproxy(\encvec_j^{\top} \cov \encvec_j) \geq \sum\limits_{j=1}^{\ipdim} \rateproxy \left( \nu_j \right) = \sum\limits_{j=1}^{d} \rateproxy(\widetilde{\encvec}_j^{\top} \cov \widetilde{\encvec}_i). $$
$$ \rateproxy\left( \left \lbrace \encvec_j^{\top} \cov \encvec_j \right \rbrace_{j=1}^{\ipdim} \right) \geq  \rateproxy \left( \left \lbrace \nu_j \right \rbrace_{j=1}^{\ipdim} \right) = \rateproxy \left( \left \lbrace \widetilde{\encvec}_j^{\top} \cov \widetilde{\encvec}_i \right \rbrace_{j=1}^{\ipdim} \right). $$
Therefore, if $\rateproxy$ is Schur-concave, the rate constraint can only improve. This implies an optimal solution can be attained when 
    $\encnew$ is such that $\encnew^{\top} \cov \encnew$ is diagonal. If $\rateproxy$ is strictly Schur-concave, the rate constraint strictly improves implying that the optimal $\encnew$ must be such that $\encnew^{\top} \cov \encnew$ is diagonal.
% since for every choice of $\encnew$, there exists a choice of $\diagenc$ such that $\diagenc^{\top} \cov\diagenc$ is diagonal and improves the constraints.
 This implies that
 \begin{align*}
\tr\left( \cov \encnew \left( \encnew^{\top} \cov \encnew + \noisevar\ide \right)^{-1} \encnew^{\top} \cov \right)  &= \tr\left(  \encnew^{\top} \cov^2 \encnew \left( \encnew^{\top} \cov \encnew + \noisevar\ide \right)^{-1}\right) \\
&= \sum\limits_{i=1}^{d} \frac{\encvec_i^{\top} \cov^2 \encvec_i}{\noisevar + \encvec_i^{\top} \cov \encvec_i}.
\end{align*}   

Note that minimizing the objective in \eqref{eq:MASTEROPTI_MMSE} is equivalent to maximizing the above expression. Perform the change of variable 
    \begin{align*}
        \encvec_j & \mapsto \begin{cases} 
            \left(\frac{\cov^{1/2} \encvec_j}{||\cov^{1/2} \encvec_j||}, ||\cov^{1/2} \encvec_j||^2\right) & \text{if $\cov^{1/2} \encvec_j \ne \bm{0}$} \\
        (\bm{0},0) & \text{if $\cov^{1/2} \encvec_j = \bm{0}$}
    \end{cases}  \\
        &  = (\var_j,y_j).
    \end{align*}
The assumption that $\encnew^\top \cov \encnew$ is diagonal and
the normalization in the definition of $\var_j$ implies that 
\[
    \vort = [ \var_1 \var_2, \cdots, \var_d]
\]
is a matrix whose nonzero columns form an orthonormal set. Rewriting the objective in terms of
the $(\var_j,y_j)$, we have

\begin{equation}\label{eq:objinY}
\sum\limits_{i=1}^{d} \frac{\encvec_i^{\top} \cov^2 \encvec_i}{\noisevar + \encvec_i^{\top} \cov \encvec_i} = \sum\limits_{i=1}^{d} \var_i^{\top} \cov \var_i \frac{y_i}{\noisevar + y_i} = \sum\limits_{i=1}^{d} \var_i^{\top} \cov \var_i m_i,
\end{equation}	
where  $m_i = \frac{y_i}{\noisevar+y_i}$. 
Observe that under this new parametrization, the constraint only depends on $\{y_i \}_{i=1}^{d}$. Without loss of generality, we assume that $y_1 \geq y_2 \geq \cdots \ge y_d$, implying that $m_1 \geq m_2 \geq \cdots \geq m_d$.
We now prove that for given $\{y_i \}_{i=1}^{d}$, choosing the $\var_i$ along the eigenvectors of $\cov$ is optimal.

%Then we have
%\begin{equation}\label{eq:OBJECTIVEORTHO}
% \sum\limits_{i=1}^{d} \frac{\var_i^T \cov \var_i}{\noisevar + y_i} = \sum\limits_{i=1}^{d} \frac{\var_i^T \cov \var_i}{y_i} m_i = \sum\limits_{i=1}^{d} \vortvec_i^{\top} \cov \vortvec_i m_i .
%\end{equation}

Denote the diagonal elements of $\vort^\top \cov \vort$ by $\{\lambda_i^2\}_{i = 1}^d$ and let  $\{ \lambda_{i, \downarrow}^2 \}_{i=1}^{d}$  denote the same diagonal elements arranged in descending order. Denote the eigenvalues of $\vort^{\top} \cov \vort$ by $\{ \orthvar_i^2 \}_{i=1}^{d}$ where $\orthvar_1 \geq \orthvar_2 \geq \cdots \geq \orthvar_d$. 
Again invoking the Schur-Horn theorem, the eigenvalues of $\vort^{\top} \cov \vort$
 majorize its diagonal entries
\begin{equation}\label{eq:majorization}
\left \lbrace \lambda_i^2 \right \rbrace_{i=1}^{d} \prec \left \lbrace \orthvar_i^2 \right \rbrace_{i=1}^{d}.
\end{equation} 
 Substituting $\lambda_i^2 = \var_i^{\top} \cov \var_i$ in \eqref{eq:objinY}, we have
\begin{align*}
\sum\limits_{i=1}^{d} \lambda_i^2 m_i \stackrel{(a)}{\leq} \sum\limits_{i=1}^{d} \lambda_{i,\downarrow}^2 m_i  &= \lambda_{1,\downarrow}^2 m_1 + \sum\limits_{i=2}^{d} \left( \sum\limits_{j=1}^{i} \lambda_{j,\downarrow}^2 -\sum\limits_{j=1}^{i-1} \lambda_{j,\downarrow}^2 \right) m_i \\
&= \lambda_{1,\downarrow}^2 m_1 +  \sum\limits_{i=2}^{d} m_i \sum\limits_{j=1}^{i} \lambda_{j,\downarrow}^2 - \sum\limits_{i=2}^{d} m_i  \sum\limits_{j=1}^{i-1} \lambda_{j,\downarrow}^2 \\
&=  \lambda_{1,\downarrow}^2 (m_1 - m_2) + m_d \left( \sum\limits_{j=1}^{d} \lambda_{j,\downarrow}^2 \right) + \sum\limits_{i=2}^{d-1} \left( m_i - m_{i+1}\right) \sum\limits_{j=1}^{i} \lambda_{j,\downarrow}^2 \\ 
&\stackrel{(b)}{\leq} \orthvar_1^2 (m_1 - m_2) + m_d \left( \sum\limits_{j=1}^{d} \orthvar_j^2 \right) + \sum\limits_{i=2}^{d-1} (m_i - m_{i+1}) \sum\limits_{j=1}^{i} \orthvar_j^2\\
 &\stackrel{(c)}{\leq} \sigma_1^2 (m_1 - m_2) + m_d \left( \sum\limits_{j=1}^{d} \sigma_j^2 \right) + \sum\limits_{i=2}^{d-1} (m_i - m_{i+1}) \sum\limits_{j=1}^{i} \sigma_j^2\\
&= \sum\limits_{i=1}^{d} \sigma_i^2 m_i,
\end{align*}

where inequality $(a)$ follows from the assumption that $m_1 \geq m_2 \geq \cdots \geq m_d$, and $(b)$ from the definition in \eqref{eq:majorization}. Since $\vort $'s nonzero columns form an orthonormal set, the eigenvalues of $\vort^{\top} \cov \vort$, when arranged in descending order, are at most the eigenvalues of $\cov$ from Corollary 4.3.37 in \cite{HornJ85}, and therefore $(c)$ follows.

This upper bound is attained when $\var_i = \eigvec_i$ for nonzero $y_i$, where $\eigvec_i$ is the normalized eigenvector of $\cov$ corresponding to eigenvalue $\sigma_i^2$. To see this, note that when $\var_i = \eigvec_i$, $\lambda_i^2 = \orthvar_i^2 = \sigma_i^2$. From the definition of $\var_i, \encvec_i = \cov^{-1/2}\eigvec_i \sqrt{y_i} = \eigvec_i \frac{\sqrt{y_i}}{\sigma_i}$. Therefore, for a Schur-concave $\rateproxy$, the set of matrices whose nonzero columns are eigenvectors of $\cov$ is optimal. We now prove that for a strictly Schur-concave $\rateproxy$, if $\cov$ has distinct eigenvalues, this set contains all of the optimal solutions $\encnew$.

%We know that for a fixed $y_1 \geq y_2 \geq \cdots y_d$, (implying a fixed $m_1 \geq m_2 \geq \cdots m_d$) the upper bound $\sum\limits_{i=1}^{d} \sigma_i^2 m_i$ can be attained by the previous choice of $\var_i$. Note that if all nonzero $m_i$ are distinct, equality in $(b)$ is attained if and only if the diagonal elements of $\vort^{\top} \cov \vort$ are the same as its eigenvalues. This implies that, if all nonzero $m_i$ are distinct, the upper bound is attained if and only if $\var_i = \eigvec_i$ for nonzero $y_i$. Therefore, it is sufficient to prove that for the following optimization problem

We know that for a fixed $y_1 \geq y_2 \geq \cdots \geq y_d$, (implying a fixed $m_1 \geq m_2 \geq \cdots \geq m_d$) the upper bound $\sum\limits_{i=1}^{d} \sigma_i^2 m_i$ is attained by the previous choice of $\var_i$. Note that if all nonzero $m_i$ are distinct, equality in $(b)$ and $(c)$ is attained if and only if the nonzero diagonal elements of $\vort^{\top} \cov \vort$ equal the corresponding eigenvalues of $\cov$. This implies that, if all nonzero $m_i$ are distinct, the upper bound is attained if and only if $\var_i = \eigvec_i$ for nonzero $y_i$. Therefore, it is sufficient to prove that for the following optimization problem

\begin{equation} \label{eq:ubschur}
\begin{aligned} 
\sup\limits_{\{y_i \geq 0\}} \quad & \sum\limits_{i=1}^{d} \sigma_i^2 \frac{y_i}{\noisevar + y_i}  \\
\text{subject to} \quad & R \geq \rho\left(\left\{y_i \right\}_{i= 1}^d\right),
\end{aligned}
\end{equation}
any optimal $\{y_i\}$ must be such that the nonzero $y_i$ are distinct. Firstly, note that since $\sigma_1^2 > \sigma_2^2 > \cdots > \sigma_d^2$, we must have $y_1 \geq y_2 \geq \cdots \geq y_d$. Assume to the contrary that for an optimal $\{ y_i \}_{i=1}^{d}$ there exists $1 \leq j, \ell < d$ such that $y_{j-1} > y_j = y_{j+1} = y_{j+2} = \cdots = y_{j+\ell} > y_{j+\ell+1} \geq 0$, where $y_0$ is chosen to be any real number strictly greater than $y_1$ and $y_{d+1}=0$. 
%Define $\delta \triangleq \min\left( \frac{y_{j-1} - y_j}{3}, \frac{y_{j+\ell}-y_{j+\ell+1}}{3}, \frac{\sigma_j^2 - \sigma_{j+\ell}^2}{\sigma_j^2 + \sigma_{j+\ell}^2} \left( \noisevar + y_j \right)\right) > 0$. 
Take $\delta > 0$ small.
Denote a new sequence $ \{ y'_i \}_{i=1}^{d}$ where $y'_{j} = y_j+\delta, y'_{j+\ell} = y_{j+\ell} - \delta$ and $y'_i = y_i$ for $1\leq i \leq d$ with $i \neq j$ and $j+\ell$. 
%\[ \{y'_i \}_{i=1}^{d} \succ \{y_i \}_{i=1}^{d}. \]
Since $\rateproxy$ is strictly Schur-concave, the constraint is strictly
improved,
\[ \rateproxy\left(  \{y'_i \}_{i=1}^{d} \right) < \rateproxy\left(  \{y_i \}_{i=1}^{d} \right). \]
Since $\sigma^2_j > \sigma^2_{j + \ell}$,  the objective is strictly
improved for sufficiently small $\delta$,
$$
\sum\limits_{i=1}^{d} \sigma_i^2 \frac{y_i}{\noisevar + y_i} <
\sum\limits_{i=1}^{d} \sigma_i^2 \frac{y'_i}{\noisevar + y'_i},
$$
as desired.
\begin{comment}
%We know that for a fixed $y_1 \geq y_2 \geq \cdots y_d$, (implying a fixed $m_1 \geq m_2 \geq \cdots m_d$) the upper bound $\sum\limits_{i=1}^{d} \sigma_i^2 m_i$ can be attained by the previous choice of $\var_i$. Note that if all nonzero $m_i$ are distinct, equality in $(b)$ is attained if and only if the diagonal elements of $\vort^{\top} \cov \vort$ are the same as its eigenvalues. This implies that, if all nonzero $m_i$ are distinct, the upper bound is attained if and only if $\var_i = \eigvec_i$ for nonzero $y_i$. Therefore, it is sufficient to prove that for the following optimization problem

%\begin{equation} \label{eq:ubschur}
%\begin{aligned} 
%\sup\limits_{\{m_i \geq 0\}} \quad & \sum\limits_{i=1}^{d} \sigma_i^2 m_i  \\
%\text{subject to} \quad & R \geq \rho\left(\left\{m_i \right\}_{i= 1}^d\right),
%\end{aligned}
%\end{equation}

the optimal nonzero $m_i$ are distinct. Firstly, note that since $\sigma_1^2 \geq \sigma_2^2 \geq \cdots \sigma_d^2$, $m_1 \geq m_2 \geq \cdots m_d$. Assume to the contrary that for an optimal $\{ m_i \}_{i=1}^{d}$ there exists $1 \leq j, \ell < d$ such that $m_{j-1} > m_j = m_{j+1} = m_{j+2} \cdots m_{j+\ell} > m_{j+\ell+1} \geq 0$, where $m_0$ is chosen to be any real number strictly greater than $m_1$ and $m_{d+1}=0$. Define $\delta \triangleq \min\left( \frac{m_{j-1} - m_j}{3}, \frac{m_{j+\ell}-m_{j+\ell+1}}{3} \right) > 0$. Denote a new sequence $ \{ m'_i \}_{i=1}^{d}$ where $m'_{j} = m_j+\delta, m'_{j+\ell} = m_{j+\ell} - \delta$ and $m'_i = m_i$ for $1\leq i \leq d$, $i \neq j,j+\ell$. Note that 
\[ \{m'_i \}_{i=1}^{d} \succ \{m_i \}_{i=1}^{d}. \]

Since $\rateproxy$ is strictly Schur-concave, 
\[ \rateproxy\left(  \{m'_i \}_{i=1}^{d} \right) < \rateproxy\left(  \{m_i \}_{i=1}^{d} \right). \]
Also  $\sigma_j^2 m'_j + \sigma_{j+\ell}^2 m'_{j+\ell} = \sigma_j^2 m_j + \sigma_{j+\ell}^2 m_{j+\ell} + \delta\left(\sigma_j^2 - \sigma^2_{j+\ell}\right) \geq  \sigma_j^2 m_j + \sigma_{j+\ell}^2 m_{j+\ell}. $ Therefore, the objective only increases while the rate constraint strictly improves, contradicting the optimality assumption. This implies that the optimal nonzero $m_i$ are distinct, further implying that for a strictly Schur-concave $\rateproxy$, the optimal value is attained only when a nonzero $\var_i = \frac{\cov^{1/2} \encvec_i}{\left \lVert \cov^{1/2} \encvec_i \right \rVert} = \eigvec_i$. Therefore, $\encvec_i = \cov^{-1/2}\eigvec_i \sqrt{y_i} = \eigvec_i \frac{\sqrt{y_i}}{\sigma_i}$. 
\end{comment}
%Note that the upper bound on the right hand side is attained when $\var_i$ are aligned along the eigenvectors of $\cov$ i.e., $\frac{\cov^{1/2}\encvec_i}{y_i} = \eigvec_i$ (and we have that $\encnew^\top \cov \encnew$ is diagonal, as required). This in turn implies that $\encvec_i = y_i\cov^{-1/2} \eigvec_i = y_i\eigmat \diagcov^{-1/2} \eigmat^T \eigvec_i$ where $\diagcov$ is the diagonal matrix whose diagonal entries are $\sigma_i^2$. Simplifying the right hand side gives $\encvec_i = \eigvec_i \frac{y_i}{\sigma_i}$. Therefore the columns $\encnew$ can be chosen to be the eigenvectors of $\cov$. Further if $\rateproxy$ is strictly concave, $\encnew$ must be of this form.
%This implies we can write the optimal encoder $\encnew^* = \eigmat \diagenc^*$ where $\diagenc^*$ is a diagonal matrix and $\eigmat$ is the matrix formed from the eigenvectors of $\cov$.
% Substituting in the right hand side of \eqref{eq:objinY}, we get 
%\[ \sum\limits_{i=1}^{d} \frac{Y_i^T \cov Y_i}{1 + \left \lVert Y_i \right \rVert_2^2} = \sum_{i=1}^{d} \frac{\sigma_i^4 \left \lVert \encnew_i \right \rVert_2^2}{1+\sigma_i^2 \left \lVert \encnew_i \right \rVert_2^2}. \]
\end{proof}

As a consequence of Theorem~\ref{thm:diagisoptimal}, encoding via an optimal $\encnew$ can be viewed as a projection along the eigenvectors of $\cov$, followed by different scalings applied to each component, i.e. $\encnew  = \eigmat \scalemat$ where $\scalemat$ is a diagonal matrix with entries $\scaling_i \geq 0$ and 
$\eigmat$ is the normalized eigenvector matrix. Only $\scalemat$ remains to be determined, and to this end, we may assume that
$\cov$ is diagonal with nonincreasing diagonal entries, implying $\eigmat = \bm{I}$. In subsequent sections, our choice of $\rateproxy$ will be of the form $\sum\limits_{i=1}^{d} \rateproxy_{sl}$, where $\rateproxy_{sl}: \RR_{\geq 0} \rightarrow \RR_{\geq 0}$\footnote{``sl" stands for single-letter} is (strictly) concave, making $\rateproxy$ (strictly) Schur-concave (see Proposition~\ref{prop:single-letter} in Appendix~\ref{app:schur}). Therefore,  \eqref{eq:MASTEROPTI_MMSE} reduces to
%For the rest of the paper, we shall assume that the empirical covariance matrix $\cov$ is diagonal since a covariance matrix can be made diagonal by an orthogonal basis transformation without changing the optimization problem. For a diagonal covariance matrix, we know $\eigmat = \ide$ and only $\scalemat$ remains to be determined. Substituting the above in \eqref{eq:MASTEROPTI_MMSE} yields an optimization problem in $\scalemat$

\begin{equation} \label{eq:MASTEROPTI_S}
\begin{aligned} 
\inf\limits_{\scalemat} \quad & \tr(\cov) - \tr(\cov \scalemat (\scalemat^{\top} \cov \scalemat + \noisevar\bm{I} )^{-1}\scalemat^{\top} \cov ) \\
\text{subject to} \quad & R \geq \rateproxy_{sl}\left( \{\scaling_i^2 \sigma^2_i \} \right),
\end{aligned}
\end{equation}
where the infimum is over diagonal matrices $\scalemat$. To handle situations for which 
\begin{equation}
    \lim_{s \rightarrow \infty} \rateproxy_{sl}(s) < \infty,
\end{equation}
we allow the diagonal entries of $\scalemat$ to be $\infty$, with the objective for such cases defined via its continuous extension.

In the next section, we will solve \eqref{eq:MASTEROPTI_S} for several specific choices of $\rateproxy_{sl}$.


==> pba-tex 2/organization.tex <==
%\subsection{Organization}

\textbf{Notation.} We denote matrices by bold capital letters e.g. $\genmat$, and vectors by bold small, e.g. $\genvec$. The $j^{\text{th}}$ column of a matrix $\genmat$ is denoted by $\genmatvec_j$ and the $j^{\text{th}}$ entry of a vector $\genvec$ by $\left[\genvec\right]_j$. We denote the set $\left \lbrace 1,2, \cdots \ipdim \right \rbrace$ by $\left[ \ipdim \right]$. A sequence $a_1, a_2, \cdots a_n$ is denoted by $\{a_i\}_{i=1}^{n}$. We denote the zero column by $\bm{0}$. Logarithms without specified bases denote natural logarithms.

\textbf{Organization.} The balance of the paper is organized as follows. We describe our constrained linear autoencoder framework in Section~\ref{sec:FRAMEWORK}. This results in an optimization problem that we solve for any Schur-concave constraint in Section~\ref{subsec:PROOF}. In Section~\ref{sec:PBAPCA}, we recover linear autoencoders and PBA under our framework. We apply the PBA solution to a problem in variable-rate compression of Gaussian sources in Section~\ref{sec:VARIABLE}. Section~\ref{sec:EXPERIMENTS} contains experiments comparing the performance of the PBA-based fixed-rate compressor against existing fixed-rate linear compressors on image and audio datasets.


==> pba-tex 2/pbca.tex <==
\section{Explicit Solutions: Conventional Linear Autoencoders and PBA} \label{sec:PBAPCA}
\subsection{Conventional Linear Autoencoders} \label{subsec:PCA}

Given a centered dataset $\data_1, \data_2, \cdots, \data_n \in \RR^{d}$, consider a linear autoencoder optimization problem where the encoder and decoder, $\encnew$ and $ \decnew$, respectively, are $d$-by-$k$ matrices where $k \leq d$ is a parameter. The goal is to minimize the mean squared error as given by \eqref{eq:1stmse}. PCA corresponds to the global optimal solution of this optimization problem, where $\encnew = \decnew = \eigmat_k$, where $\eigmat_k \in \RR^{d \times k}$ is a matrix whose columns are the $k$ eigenvectors corresponding to the $k$ largest eigenvalues of $\cov$. However, there are multiple global optimal solutions, given by any encoder-decoder pair of the form $\left( \eigmat_k  \bm{V},  \eigmat_k  \bm{V} \right)$, where $\bm{V}$ is an orthogonal matrix \cite{BaldiH89}. 




%Consider the linear autoencoder setup in Section~\ref{sec:FRAMEWORK} where our goal was to design $\encnew$ and $\decnew$ to minimize the mean squared error when the latent variables $\encnew^{\top} x$ are quantized, subject to a Schur-concave constraint on the latent variances. A linear dimensionality reduction algorithm seeks to minimize the mean squared error subject to restricting the dimension of the latent space, i.e., subject to $\encnew, \decnew \in \RR^{d \times k}$, where $k \in \NN, k \leq d$ is a parameter. PCA is a linear dimensionality reduction algorithm that uses $\encnew = \decnew =  \eigmat_k$, where $\eigmat_k \in \RR^{d \times k}$ is a matrix whose columns are the $k$ eigenvectors corresponding to the $k$ largest eigenvalues of $\cov$. 

%Note that, unlike the linear dimensionality reduction framework, in Section~\ref{sec:FRAMEWORK}, the latent variables $\encnew^{\top} \data$ are quantized. Therefore, an infinite value of $\scaling_i$ indicates sending $\eigvec_i^{\top} \data$ with full precision where $\eigvec_i$ is the eigenvector corresponding to the $i^{th}$ largest eigenvalue. This implies that PCA with parameter $k$ corresponds to $\encnew = \eigmat \scalemat$, where 
%\begin{equation}\label{eq:PCA_S}
%    \scalemat = \left[ \begin{array}{ccccccc}
%        \infty & &  & &  &  &   \\
%         & \infty &  &  &  &  &   \\
%         &  & \ddots &  &  &  &   \\
%         &  &  & \infty &  &  &   \\
%        &  & &  & 0 &  &   \\
%         &  &  &  &  & \ddots &   \\
%         &  &  &  &  &  & 0  \\
%         \end{array} \right],
%\end{equation}
%has $k$ infinite values.


We now recover linear autoencoders through our framework in Section~\ref{sec:FRAMEWORK}. Consider the optimization problem in \eqref{eq:MASTEROPTI_S} where $\rateproxy_{sl}: \RR_{\geq 0} \rightarrow \{0,1 \}$ is a concave function defined as
\begin{equation} \label{eq:PCA_F}
\rateproxy_{sl}(x) = \bm{1} \left[ x > 0 \right].
\end{equation}

Note that this penalizes the dimension of the latents, as desired.
Note also that this cost is Schur-concave but not strictly so.
The fact that PCA solves conventional linear autoencoding,
but is not necessarily the unique solution, follows immediately
from Theorem~\ref{thm:diagisoptimal}.

\begin{theorem}\label{thm:PCA}
    If $\rateproxy_{sl}(\cdot)$ is given by \eqref{eq:PCA_F}, then an optimal solution for \eqref{eq:MASTEROPTI_S} is given by a diagonal matrix $\scalemat$ whose top $\min(\lfloor R \rfloor, d)$ diagonal entries are equal to $\infty$ and the remaining entries are $0$.
\end{theorem}
\begin{proof}
%Note that since $\rateproxy$ is bounded, we would need to take the limiting case as the scalings tend to infinity. By Theorem~\ref{thm:diagisoptimal} and the assumption that $\cov$ is diagonal, $\encunit = \ide$. We now find the scalings that we denote by $\left \lbrace w_i \right \rbrace$. 
Let $\cF \ed \left \lbrace i \in \left[ \ipdim \right] : \scaling_i > 0 \right \rbrace$, implying $\left \lvert \cF \right \rvert \leq R$. Since $\cov$ and $\scalemat$ are diagonal, the optimization problem in \eqref{eq:MASTEROPTI_S} can be written as 

\begin{equation} \label{eq:PCA_OPT}
\begin{aligned} 
\inf\limits_{\left \lbrace \scaling_{\ell} \right \rbrace} & \sum\limits_{j \in \left[d\right] \backslash \cF} \sigma_j^2 + \sum\limits_{ \ell \in \cF} \frac{\noisevar \sigma_{\ell}^2}{\noisevar+ \sigma_{\ell}^2 \scaling_{\ell}^2} \\
\text{subject to} \quad & R \geq \sum\limits_{i=1}^{d} \bm{1}\left[ \scaling_i > 0 \right].
\end{aligned}
\end{equation}

 Since the value of $\scaling_{\ell}, \ell \in \cF$ does not affect the rate constraint, each of the $\scaling_{\ell}$ can be made as large as possible without changing the rate constraint. Therefore, the infimum value of the objective is $\sum\limits_{j \in \left[ d \right] \backslash \cF} \sigma^2_j$. Since we seek to minimize the distortion, the optimal $\cF$ is the set of indices with the largest $\left \lvert \cF \right \rvert$ eigenvalues. Since the number of these eigenvalues cannot exceed $R$,  we choose $\left \lvert \cF \right \rvert = \min(\lfloor R \rfloor,d)$. 
\end{proof}

Unlike the conventional linear autoencoder framework, in Section~\ref{sec:FRAMEWORK}, the latent variables $\encnew^{\top} \data$ are quantized, which we model with additive white noise of fixed variance.  Therefore, an infinite value of $\scaling_i$ indicates sending $\eigvec_i^{\top} \data$ with full precision where $\eigvec_i$ is the eigenvector corresponding to the $i^{th}$ largest eigenvalue. This implies that PCA with parameter $k$ corresponds to $\encnew = \eigmat \scalemat$, where $\scalemat$ is a diagonal matrix whose top $k$ diagonal entries are equal to $\infty$ and the  $d-k$ remaining diagonal entries are $0$. Therefore, for any $R$ such that $\lfloor R \rfloor = k$, an optimal solution to \eqref{eq:MASTEROPTI_S} corresponds to linearly projecting the data along the top $k$ eigenvectors, which is the same as PCA. Note that, like \cite{BaldiH89}, we only prove that projecting along the eigenvectors is one of possibly other optimal solutions. However, even a slight amount of curvature in $\rateproxy$ would make it strictly Schur-concave, thus recovering the principal directions.
We next turn to a specific cost function with curvature, namely
the PBA cost function that was our original motivation.

\subsection{Principal Bit Analysis (PBA)}

Consider the choice of $\rateproxy_{sl}:\RR_{\geq 0} \rightarrow \RR_{\geq 0}$ that provided the
original impetus for Theorem~\ref{thm:diagisoptimal}. For $\gamma>\frac{2}{\sigma^2}$,

\begin{equation}\label{eq:LOG_F}
\rateproxy_{sl}(x) = \frac{1}{2} \log(\gamma x+1).
\end{equation}

The nature of the optimization problem depends on the value 
of $\gamma$. For $1 \le \gamma \sigma^2 \le 2$, the problem can be
made convex with a simple change of variable. For $\gamma \sigma^2= 1$,
the problem coincides with the classical waterfilling procedure
in rate-distortion theory, in fact. For $\gamma \sigma^2 > 2$, the problem
is significantly more challenging. Since we are interested in
relatively large values of $\gamma$ for our compression application
(see Section~\ref{sec:EXPERIMENTS} to follow), we focus on the case $\gamma > 2/\sigma^2$.

%The above choice of function is motivated by rate-distortion theory \cite{CoverT06} which states that a Gaussian source with variance $\sigma^2$ requires at least $\frac{1}{2} \log \left( \frac{\sigma^2}{D} \right)$ bits to be represented up to mean squared error of $D$.

%We now motivate the choice of our function. It can be shown that for random variables $X \sim \cN\left(0,\sigma^2\right)$ and $\eps$ such that $\EE\left[ \eps^2 \right] \leq D$ for $D>0$,  $I\left( X; X+\eps \right) \geq \frac{1}{2}\log\left( \frac{\sigma^2}{D} \right)$. From rate distortion theory \cite{CoverT06}, this mutual information can be thought of as the number of bits required to represent a quantized $X$ with a mean squared error distortion constraint of $D$. 

%\begin{comment}
%The next theorem describes a  ``reverse water-filling'' algorithm, which we call Principal Bit Analysis (PBA), that 
%computes an optimal $\scalemat$.

%\begin{algorithm}[h]
%	\caption{Principal Bit Analysis (PBA)} \label{alg:PBA}
%	\begin{algorithmic}[1]
%		\Require $R > 0$, $\cov$ - diagonal covariance matrix with diagonal elements $\sigma_i^2$, $1\leq i \leq d$ with $\sigma_1^2 \geq \sigma_2^2 \geq \cdots \geq \sigma_d^2$.
%		\State Compute $\lb_j = \frac{1}{2} \log \left( \frac{\prod\limits_{i=1}^{j} \sigma_i^2}{\sigma_j^{2j}} \right)$ for $1\leq j \leq d$ and $\lb_{d+1} = \infty$.
%		\State Find largest $\send$ such that $\lb_{\send} \leq R$. \label{line:SEND_CONDITION}
%		\State $\distortion = \frac{\sigma_{\send}^2}{2^{\frac{2\left( R - \lb_{\send} \right)}{\send}}} = \left( \frac{\prod_{i=1}^{\send} \sigma_i^2}{2^{2R}} \right)^{1/\send}$
%		
%		 \[ \distortion_i = 
%		\begin{cases} 
%		 \distortion, & \text{for } 1\leq i \leq \send, \\
%		\sigma_i^2, & \text{for } \send +1\leq i \leq \ipdim. 
%		\end{cases}
%		\]  \label{line:DISTORTION}
%		\State $\scaling_i = \sqrt{\frac{1}{D} - \frac{1}{\sigma_i^2}} \hspace{5mm} 1\leq i \leq \send$. \label{line:SCALING}
%		%\State $R_i = \frac{1}{2} \log \left( \frac{\sigma_i^2}{D}\right)  \hspace{5mm} 1\leq i \leq s \text{ and } 0 \text{ o.w}.$  \label{line:RATEALLOCATION}
%		\State Output $\scalemat = \text{diag}\left(\scaling_1, \scaling_2, \cdots \scaling_{\send}, \underbrace{0,0, \cdots 0}_{\ipdim-\send} \right)$
%	\end{algorithmic}
%\end{algorithm} 
%The key principle in PBA is the equalization of distortions across the components that send a positive rate thus resembling a reverse water-filling solution. This is not surprising since the formulation is very similar to that of the rate-distortion theorem for a parallel Gaussian source. We now prove that in fact PBA provides the optimal $\encnew$. 
%
%\begin{theorem}\label{thm:PBA}
%For $R>0$, an optimal $\scalemat$ is given by 
%\begin{equation}
%    s_i^2 = \frac{1}{D_i} - \frac{1}{\sigma^2_i},
%\end{equation}
%where
%\begin{equation}
%       D_i = \min(\lambda,\sigma^2_i) 
%\end{equation}
%    and $\lambda$ is the unique positive number such that
%\begin{equation}
%    \sum_{i = 1}^d \frac{1}{2} \log \frac{\sigma^2_i}{D_i} = R.
%\end{equation}
%\end{theorem}
%
%\begin{proof}
%Recall that in the original problem formulation we express $\encnew = \encunit \scalemat$. Since for this case, $\rateproxy$ is not bounded, the limiting case does not apply. Since $\cov$ is assumed to be diagonal, $\encunit = \ide$ and we only have to find the finite scalings. 
%Let $\scalemat = \text{diag}\left( \scaling_1, \scaling_2, \cdots \scaling_{\ipdim} \right)$. Rewriting the optimization problem in \eqref{eq:MASTEROPTI_S} with $\rateproxy$ given by \eqref{eq:LOG_F}, we have 
%
%\begin{equation} \label{eq:PBA_OPT}
%\begin{aligned} 
%\inf\limits_{\left \lbrace \scaling_i \right \rbrace} \quad & \sum\limits_{i=1}^{\ipdim} \frac{\sigma_{i}^{2}}{1+\scaling_{i}^{2} \sigma_{i}^{2}} \\
%\text{subject to } \quad & R \geq \frac{1}{2}\sum\limits_{i=1}^{d} \log(\scaling_i^2 \sigma_i^2+1).
%\end{aligned}
%\end{equation}
%Perform the change of variable Let $s_i \mapsto \distortion_i = \frac{\sigma_i^2}{1+\scaling_i^2 \sigma_i^2}$. Then the problem
%becomes
%\begin{equation}\label{eq:PBA_OPT_DISTORTION}
%\begin{aligned} 
%\inf\limits_{\left \lbrace \distortion_i \right \rbrace} \quad & \sum\limits_{i=1}^{\ipdim} \distortion_i \\
%\text{subject to} \quad & 2R \geq \sum\limits_{i=1}^{\ipdim} \log\left(\frac{\sigma_i^2}{\distortion_i}\right),\\
%&\distortion_i \leq \sigma_i^2.
%\end{aligned}
%\end{equation}
%    This is precisely the distortion-rate function of a Gaussian vector with covariance matrix $\cov$, so the conclusion follows from
%    the classical reverse waterfilling characterizatoin of this function~\cite{CoverT06??needmoreprecisereference}.
%   
%\end{proof} 
%\begin{comment}
%The Lagrangian can be written as 
%\[ \cL(\left \lbrace \distortion_i, \mu_i \right \rbrace, \lambda)  = \sum\limits_{i=1}^{\ipdim} \distortion_i + \lambda \left(\sum\limits_{i=1}^{\ipdim} \log\left(\frac{\sigma_i^2}{\distortion_i}\right) - 2R \right) + \sum\limits_{i=1}^{\ipdim} \mu_i (\distortion_i  - \sigma_i^2). \]
%For $1 \leq i \leq \ipdim$, the KKT conditions are 
%\begin{equation}\label{eq:KKTgrad}
%\frac{\partial \cL}{\partial \distortion_i} = 1 - \frac{\lambda \log_2(e)}{\distortion_i} + \mu_i = 0,
%\end{equation}
%along with the primal feasibility, dual feasibility conditions : $\lambda \geq 0, \mu_i \geq 0$ for $1 \leq i \leq \ipdim$ and  complementary slackness conditions. We show that the distortions $\left \lbrace \distortion_i \right \rbrace_{i=1}^{d}$ obtained from PBA, $\lambda = \frac{\distortion}{\log_2(e)}$, $\mu_i = 0$ for $1\leq i \leq \send$, $\mu_i = \frac{\distortion}{\sigma_i^2}-1, \send+1 \leq i \leq d$  satisfy the KKT conditions.  
%
%For $1\leq i \leq \send$, $\distortion_i = \distortion \leq \sigma_i^2$ from the definition of $\distortion$ and the fact that $R \geq \lb_{\send}$. For $\send+1\leq i \leq \ipdim$, $\distortion_i = \sigma_i^2$. The rate constraint is met with equality by definition of $\distortion$. Therefore, the distortions from PBA correspond to a primal feasible solution. Since $\distortion > 0$, $\lambda$ is dual feasible. Since $R < \lb_{\send+1}$,$2^{2R} \leq \frac{\prod\limits_{i=1}^{\send+1} \sigma_i^2}{\sigma_{\send+1}^{2(\send+1)}}$ implies $D \geq \sigma_{\send+1}^2 \geq \sigma_i^2$ for $\send+1 \leq i \leq \ipdim$.  Therefore, $\lambda, \left \lbrace \mu_i \right \rbrace_{i=1}^{\ipdim}$ are dual feasible. Since the rate constraint is met with equality, the complementary slackness is satisfied for the rate constraint. Also, since $\mu_i = 0$ for $1\leq i\leq \send$ and $\distortion_i = \sigma_i^2$ for $\send+1 \leq i \leq \ipdim$, complementary slackness is satisfied for the distortion constraints as well. Finally, we see that for $1\leq i\leq \send$, \eqref{eq:KKTgrad} is satisfied since $\mu_i=0, \lambda = \frac{\distortion}{\log_2(e)}$ and for $\send+1\leq i \leq \ipdim$, since $\lambda \log_2(e) = \distortion$, \eqref{eq:KKTgrad} is satisfied. 
%
%We can find a strictly feasible point in the domain of \eqref{eq:PBA_OPT_DISTORTION} by equalizing the rates to $\frac{R}{d}$ for a given $R>0$. Therefore by Slater's condition  strong duality holds implying that the solution provided by PBA is optimal.
%\end{comment}

%\begin{algorithm}[h]
%	\caption{Principal Bit Analysis (PBA)} \label{alg:PBA}
%	\begin{algorithmic}[1]
%		\Require  $\cov$ - diagonal covariance matrix with diagonal elements $\sigma_i^2$, $1\leq i \leq d$ with $\sigma_1^2 \geq \sigma_2^2 \geq \cdots \geq \sigma_{\ipdim}^2$.
%		\State Compute $\lb_j = \frac{1}{2} \log \left( \frac{\prod\limits_{i=1}^{j} \sigma_i^2}{\sigma_j^{2j}} \right)$ for $1\leq j \leq d$ and $\lb_{d+1} = \infty$.
%		\State Find largest $\send$ such that $\lb_{\send} \leq R$. \label{line:SEND_CONDITION}
%		\State $\distortion = \frac{\sigma_{\send}^2}{2^{\frac{2\left( R - \lb_{\send} \right)}{\send}}} = \left( \frac{\prod_{i=1}^{\send} \sigma_i^2}{2^{2R}} \right)^{1/\send}$
%		
%		 \[ \distortion_i = 
%		\begin{cases} 
%		 \distortion, & \text{for } 1\leq i \leq \send, \\
%		\sigma_i^2, & \text{for } \send +1\leq i \leq \ipdim. 
%		\end{cases}
%		\]  \label{line:DISTORTION}
%		\State $\scaling_i = \sqrt{\frac{1}{D} - \frac{1}{\sigma_i^2}} \hspace{5mm} 1\leq i \leq \send$. \label{line:SCALING}
%		%\State $R_i = \frac{1}{2} \log \left( \frac{\sigma_i^2}{D}\right)  \hspace{5mm} 1\leq i \leq s \text{ and } 0 \text{ o.w}.$  \label{line:RATEALLOCATION}
%		\State Output $\scalemat = \text{diag}\left(\scaling_1, \scaling_2, \cdots \scaling_{\send}, \underbrace{0,0, \cdots 0}_{\ipdim-\send} \right)$
%	\end{algorithmic}
%\end{algorithm} 

\begin{algorithm}[h]
	\caption{Principal Bit Analysis (PBA)} \label{alg:PBA}
	\begin{algorithmic}[1]
		\Require $\lambda > 0$, $\scalePBA  > 2$, 
		\begin{equation}
            \cov = \left[ \begin{array}{cccc}
                \sigma^2_1 & 0 & \cdots & 0 \\
                0 & \sigma^2_2 & \cdots & 0 \\
                \vdots & \vdots & \ddots & \vdots \\
                0 & 0 & \cdots & \sigma^2_\ipdim \\
            \end{array} \right] \succ 0,
            \end{equation}
		such that $\sigma^2_1 \ge \sigma^2_2 \ge \cdots \ge \sigma^2_\ipdim$.
		\State If $\lambda \ge \sigma^2_1/(4(\scalePBA - 1))$, Output  
			   $\bar{R}_{\text{opt}} = 0, \bar{D}_{\text{opt}} = \sum_{i = 1}^\ipdim \sigma^2_i$.
		\State Set $\bar{\ipdim} = \max\left\{i : \lambda < \sigma_i^2/4(\alpha - 1)\right\}$.
			\State Set $\bar{R}$, $\bar{D}$ to zero arrays of size $2\bar{\ipdim}$.
			\For{$\send \in \left \lbrace 1,2, \cdots \bar{\ipdim} \right \rbrace $}
				\State $\bar{D}(2\send-1) =  \sum\limits_{i=1}^{\send} \frac{\sigma_i^2}{2(\scalePBA -1)} \left( 1 - \sqrt{1 - \frac{4 \lambda (\scalePBA -1)}{\sigma_i^2}}\right) + \sum\limits_{i=\send+1}^{\ipdim} \frac{\sigma_i^2}{\scalePBA } $, 
				\State $\bar{R}(2\send-1)= \sum\limits_{i=1}^{\send} \frac{1}{2} \log \left( \frac{\sigma_i^2}{4\lambda} \right) + \log\left( 1 + \sqrt{1 - \frac{4 \lambda (\scalePBA -1)}{\sigma_i^2}}\right)$.
				\State $\bar{D}(2\send) =\left( \sum\limits_{i=1}^{\send-1} \frac{\sigma_i^2}{2(\scalePBA -1)} \left( 1 - \sqrt{1 - \frac{4 \lambda (\scalePBA -1)}{\sigma_i^2}}\right) + \frac{\sigma_{\send}^2}{2(\scalePBA -1)} \left( 1 + \sqrt{1 - \frac{4 \lambda (\scalePBA -1)}{\sigma_{\send}^2}}\right) + \sum\limits_{i=\send+1}^{\ipdim} \frac{\sigma_i^2}{\scalePBA } \right)$.
				\State $\bar{R}(2\send)=\sum\limits_{i=1}^{\send} \frac{1}{2} \log \left( \frac{\sigma_i^2}{4\lambda} \right) + \sum\limits_{i=1}^{\send-1} \log\left( 1 + \sqrt{1 - \frac{4 \lambda (\scalePBA -1)}{\sigma_i^2}}\right) + \log\left( 1 - \sqrt{1 - \frac{4 \lambda (\scalePBA -1)}{\sigma_{\send}^2}}\right)$.
			\EndFor
			\State $\send^* \leftarrow \argmin_{j \in \left[ 2\bar{\ipdim} \right]} \bar{D}(j) + \lambda \bar{R}(j). $
%			\State $\bar{R}_{\text{opt}}.\text{append}\left(\bar{R}(\send^*)\right), \bar{D}_{\text{opt}}.\text{append}\left(\bar{D}(\send^*)\right)$.
		\State Output $\bar{R}_{\text{opt}} = \bar{R}(\send^*), \bar{D}_{\text{opt}} = \bar{D}(\send^*)$.
			
	\end{algorithmic}
\end{algorithm} 

%\If{$\send^*$ is odd}
%				\For{$j \in \left \lbrace 1,2, \cdots \send^*\right \rbrace $}
%					\State $\scaling_j = \sqrt{\frac{1}{\frac{\sigma_j^2}{2(a-1)} \left( 1 - \sqrt{1 - \frac{4 \lambda (a-1)}{\sigma_j^2}}\right)} - \frac{a}{\sigma_j^2}}$.
%				\EndFor
%			\Else
%				\For{$j \in\left \lbrace 1,2, \cdots \send^*-1\right \rbrace$}
%						\State $\scaling_j = \sqrt{\frac{1}{\frac{\sigma_j^2}{2(a-1)} \left( 1 - \sqrt{1 - \frac{4 \lambda (a-1)}{\sigma_j^2}}\right)} - \frac{a}{\sigma_j^2}}$.
%				\EndFor
%				\State $\scaling_{\send^*} = \sqrt{\frac{1}{\frac{\sigma_{\send^*}^2}{2(a-1)} \left( 1 + \sqrt{1 - \frac{4 \lambda (a-1)}{\sigma_{\send^*}^2}}\right)} - \frac{a}{\sigma_{\send^*}^2}}$.
%			\EndIf
%		\EndFor
%		\State Output $\scalemat = \text{diag}\left(\scaling_1, \scaling_2, \cdots \scaling_{\send^*}, \underbrace{0,0, \cdots 0}_{\ipdim-\send^*} \right)$.

\begin{theorem}
If $\rateproxy_{sl}(\cdot)$ is given by \eqref{eq:LOG_F} for $\gamma > \frac{2}{\sigma^2}$, then for any $\lambda > 0$,
	the pair $\bar{R}_{\text{opt}}, \bar{D}_{\text{opt}}$ obtained from the output of 
	  Algorithm~\ref{alg:PBA} satisfies 
	  \begin{equation} 
		  \label{eq:PBA_OPT_LAGRANGE}
			   \bar{D}_{\text{opt}} + \lambda \bar{R}_{\text{opt}} = 
			  \inf\limits_{\scalemat} \quad \tr(\cov) - \tr(\cov \scalemat (\scalemat^{\top} \cov \scalemat + \noisevar\bm{I} )^{-1}\scalemat^{\top} \cov )  
			  + \lambda \sum_{i = 1}^\ipdim \rateproxy_{sl}\left( \{\scaling_i^2 \sigma^2_i \} \right),
	  \end{equation}
\end{theorem}

\begin{proof}
Since $\cov$ and $\scalemat$ are diagonal, the optimization problem in 
\eqref{eq:PBA_OPT_LAGRANGE} can be written as 
\begin{equation} \label{eq:PBA_OPT}
\begin{aligned} 
\inf\limits_{\left \lbrace \scaling_i \right \rbrace} \quad & \sum\limits_{i=1}^{d} \frac{\noisevar \sigma_{i}^{2}}{\noisevar+\scaling_{i}^{2} \sigma_{i}^{2}} 
   + \lambda \cdot \frac{1}{2}\sum\limits_{i=1}^{d} \log\left( 1 + \gamma \scaling_{i}^2 \sigma_{i}^{2} \right).
\end{aligned}
\end{equation}
With the following change of variables $ \scalePBA = \gamma \sigma^2 $, $\scaling_{i} \mapsto \scaling_{i}'^2 = \scalePBA \frac{\scaling_{i}'^2}{\sigma^2}$, we obtain 


\begin{equation} \label{eq:PBA_OPT_p1}
\begin{aligned} 
\inf\limits_{\left \lbrace \scaling_i' \right \rbrace} \quad & \sum\limits_{i=1}^{d} \scalePBA \frac{ \sigma_{i}^{2}}{\scalePBA+\scaling_{i}^{'2} \sigma_{i}^{2}}  + \lambda \cdot \frac{1}{2}\sum\limits_{i=1}^{d} \log\left( 1 + \scaling_i'^2 \sigma_{i}^{2} \right).
\end{aligned}
\end{equation}

Ignoring the constant factor in the objective, perform the change of variable $\scaling'_{i} \mapsto \distortion_i = \frac{\sigma_i^2}{\scalePBA  +\scaling_{i}'^2\sigma_{i}^{2}}$
to obtain
\begin{equation} \label{eq:PBA_REDUCED_OPT}
\begin{aligned} 
\inf\limits_{\left \lbrace \distortion_i \right \rbrace} \quad & \sum\limits_{i=1}^{\ipdim} \distortion_i  + \frac{\lambda}{2}\sum\limits_{i=1}^{d} \log\left( \frac{\sigma_i^2}{\distortion_i} - (\scalePBA -1) \right), \\
    \text{subject to} \quad &\distortion_i \leq \frac{\sigma_i^2}{\scalePBA } \hspace{5mm} \text{ for all } i \in \left[ \ipdim \right].
\end{aligned}
\end{equation}

This optimization problem is nonconvex since the function $\log\left( \frac{\sigma_i^2}{\distortion_i} - (\scalePBA -1) \right)$ is convex for $0 \leq \distortion_i \leq \frac{\sigma_i^2}{2(\scalePBA -1)}$ but concave for $\frac{\sigma_i^2}{2(\scalePBA -1)} < \distortion_i \leq \frac{\sigma_i^2}{\scalePBA}$ and the
latter interval is nonempty since $\scalePBA>2$. 

	Any optimizing $\{\distortion_i\}$ must be a stationary point of 
\begin{equation}\label{eq:LAG_PBA}
\lag\left( \setD, \lambda, \setmu \right) = \sum\limits_{i=1}^{\ipdim} \distortion_i + \lambda\left( \sum\limits_{i=1}^{\ipdim} \log\left( \frac{\sigma_i^2}{\distortion_i} - (\scalePBA -1) \right) \right) + \sum\limits_{i=1}^{\ipdim} \mu_i \left( \distortion_i - \frac{\sigma_i^2}{\scalePBA } \right). 
\end{equation}
for some $\{\mu_i\}_{i = 1}^\ipdim$ with $\mu_i \geq 0$ for all $i \in \left[ \ipdim \right]$ and satisfying the complementary slackness condition~\cite[Prop.~3.3.1]{Bertsekas:Nonlinear}.  The stationary points satisfy, for each $i$
\begin{equation}\label{eq:LAG_STAT}
\frac{\partial \lag}{\partial \distortion_i} = 1 - \lambda\left( \frac{\frac{\sigma_i^2}{\distortion_i^2}}{\left( \frac{\sigma_i^2}{\distortion_i} - (\scalePBA -1) \right)}\right) + \mu_i = 0.
\end{equation}

%From \eqref{eq:PBA_REDUCED_OPT}, the rate constraint is met with equality since otherwise decreasing any $\distortion_i$ results in a smaller objective while still being in the feasible region. 
	Let $\cF = \left \lbrace i : \distortion_i < \frac{\sigma_i^2}{\scalePBA } \right \rbrace$. 
    %For $i \notin \cF$, $\distortion_i = \frac{\sigma_i^2}{\scalePBA }$. 
 For $i \in \cF$, $\mu_i = 0$ due to complementary slackness. Substituting in \eqref{eq:LAG_STAT} we obtain a quadratic equation in $\distortion_i$
 
 \[
 (\scalePBA-1)\distortion_i^2 - \sigma_i^2 \distortion_i + \lambda \sigma_i^2 = 0. 
 \]
 which gives 
 $$ \distortion_i = \frac{\sigma_i^2}{2(\scalePBA -1)} \left( 1 \pm \sqrt{1 - \frac{4\lambda (\scalePBA -1)}{\sigma_i^2}} \right).$$

Let $c_i = \sqrt{1 - \frac{4\lambda (\scalePBA -1)}{\sigma_i^2}}$. Note that $\frac{\sigma_i^2}{2(\scalePBA -1)} \left( 1 + c_i \right)$ is always in the concave region and $\frac{\sigma_i^2}{2(\scalePBA -1)} \left( 1 - c_i \right)$ is always in the convex region for a $\lambda$ chosen such that $\distortion_i$ is a real number strictly less than $\frac{\sigma_i^2}{\scalePBA }$. 

%Note that for $\distortion_i$ to be a real number, $\lambda \leq \frac{\sigma_i^2}{4(a-1)}$. Also since $i \in \cF$, $\distortion_i < \frac{\sigma_i^2}{a}$ implying

Therefore the optimal set of distortions are contained in the following set of $3^{\ipdim}$ points 
$$ \prod_{i = 1}^\ipdim \left\{   \frac{\sigma_i^2}{2(\scalePBA -1)} \left( 1 + \sqrt{1 - \frac{4\lambda (\scalePBA -1)}{\sigma_i^2}} \right),  \frac{\sigma_i^2}{2(\scalePBA -1)} \left( 1 - \sqrt{1 - \frac{4\lambda (\scalePBA -1)}{\sigma_i^2}} \right), \frac{\sigma_i^2}{\scalePBA}\right\}.$$

We now reduce the size of the above set by making a two observations:

%\noindent\textbf{$\cF$ is contiguous} 
%\begin{lemma}
%For $R>0$, let $\left \lbrace \distortion_i^* \right \rbrace_{i=1}^{d}$ be an optimal solution for \eqref{eq:PBA_REDUCED_OPT}. $\cF = \left \lbrace i : \distortion_i^* < \frac{\sigma_i^2}{a} \right \rbrace$ is $\left[ | \cF | \right]$.
%
%\end{lemma}
%\begin{proof}
%Assume to the contrary that there exist $i,j$ such that $j \in \cF, i \notin \cF$ and $j > i$. Denote $\distortion_j^* = \gamma \frac{\sigma_j^2}{a}$ where $\gamma < 1$. Since $i \notin \cF$, $\distortion_i^* = \frac{\sigma_i^2}{a}$. The rate contributions from these components combined is $\log\left( \frac{a}{\gamma} - (a-1)\right)$ and $\distortion_i^* + \distortion_j^* = \frac{\sigma_i^2}{a} + \gamma \frac{\sigma_j^2}{a}$. Let $\left \lbrace \distortion_{\ell}^{'} \right \rbrace_{\ell=1}^{\ipdim}$ be such that $\distortion_j^{'} = \frac{\sigma_j^2}{a}$, $\distortion_i^{'}= \gamma \frac{\sigma_i^2}{a}, \distortion_{\ell}^{'} = \distortion_{\ell}^*$ for $\ell \in \left[ \ipdim \right], \ell \neq i,j$. Note that the new rate is same as the optimal solution rate but $\distortion_i^{'} + \distortion_j^{'}  = \gamma\frac{\sigma_i^2}{a} + \frac{\sigma_j^2}{a} \leq \distortion_i^* + \distortion_j^*$.  Therefore $\left \lbrace \distortion_{\ell}^{'} \right \rbrace_{\ell=1}^{\ipdim}$ results in a lower distortion than the optimal solution while the rate is constant. This is a contradiction, implying that, if $j \in \cF, i \notin \cF$ then $j < i$. Therefore $\cF = \left[ | \cF | \right]$.
% \end{proof}

\noindent \textbf{(1). $\cF$ is contiguous.} 


\begin{lemma}\label{lem:NORM_INC}
There exists an optimal $\left \lbrace \distortion_i^* \right \rbrace_{i=1}^{d}$ for \eqref{eq:PBA_REDUCED_OPT} such that (a) $\frac{\sigma_i^2}{\distortion_i^*}$ is a nonincreasing sequence and (b) $\cF = \{ 1,2,\cdots \left \lvert \cF \right \rvert \}$. 
\end{lemma}

\begin{proof}
Substitute $x_i = \frac{\sigma_i^2}{\distortion_i}$ in \eqref{eq:PBA_REDUCED_OPT}. This gives us 
\begin{equation} \label{eq:PBA_NORM_OPT}
\begin{aligned} 
\inf\limits_{\left \lbrace x_i \right \rbrace} \quad & \sum\limits_{i=1}^{\ipdim} \frac{\sigma_i^2}{x_i} + \frac{\lambda}{2}\sum\limits_{i=1}^{d} \log\left( x_i - (\scalePBA -1) \right), \\
    \text{subject to} \quad & x_i \geq \scalePBA \hspace{5mm} \text{ for all } i \in \left[ \ipdim \right].
\end{aligned}
\end{equation}
Let $\{ x_i^* \}_{i=1}^{d}$ be an optimal solution for \eqref{eq:PBA_NORM_OPT}. If, for $i>j$, $x_i^* > x_j^* \ge \scalePBA$, then exchanging the values provides a solution that has the same rate and lower distortion since $\frac{\sigma_i^2}{x_i^*} + \frac{\sigma_j^2}{x_j^*} \geq \frac{\sigma_i^2}{x_j^*} + \frac{\sigma_j^2}{x_i^*}$. This proves (a). Part (b) follows immediately.
%
%For $i \in \cF$, $\distortion_i^* < \frac{\sigma_i^2}{\scalePBA }$ implies $x_i^* > \scalePBA $. This implies $\cF  = \{1,2, \cdots \left \lvert \cF \right \rvert \}$.
\end{proof}

 
\noindent\textbf{(2). No two solutions are concave.}
\begin{lemma}\label{lem:SINGLE_CONCAVE}
For $R>0$, let $\left \lbrace \distortion_i^* \right \rbrace_{i=1}^{\ipdim}$ be an optimal solution for \eqref{eq:PBA_REDUCED_OPT}. There exists at most one $\distortion_i^*$ such that $\frac{\sigma_i^2}{2(\scalePBA -1)} < \distortion_i^* < \frac{\sigma_i^2}{\scalePBA }$.
\end{lemma}

\begin{proof}
Let $\distortion_i^*, \distortion_j^*$ be such that $\frac{\sigma_i^2}{2(\scalePBA -1)} < \distortion_i^* < \frac{\sigma_i^2}{\scalePBA }$ and $\frac{\sigma_j^2}{2(\scalePBA -1)} < \distortion_j^* < \frac{\sigma_j^2}{\scalePBA }$ . Without loss of generality, assume $\distortion_i^* < \distortion_j^*$. Denote the individual rate constraint function by $r\left( \distortion_i \right) \triangleq \log \left( \frac{\sigma_i^2}{\distortion_i} - (\scalePBA -1) \right)$. Since $r$ is concave in $\left(\frac{\sigma_i^2}{2(a-1)}, \frac{\sigma_i^2}{\scalePBA } \right)$, there exist an $\eps > 0$ such that

\begin{align}
r\left(\distortion_i^* - \eps\right) +r\left( \distortion_j^* + \eps \right) &=  r\left( \distortion_i^* \right) - \eps r'\left( \distortion_i^* \right) + O(\eps^2) + r\left(\distortion_j^*\right) + \eps r'\left(\distortion_j^* \right) + O(\eps^2) \\
 &< r\left( \distortion_i^* \right) + r\left(\distortion_j^*\right)
\end{align}
The last inequality follows from concavity of $r$. Therefore,  replacing $\left(\distortion_i^*, \distortion_j^*\right)$ with $\left(\distortion_i^* - \eps, \distortion_j^*+ \eps \right)$, the rate constraint can be improved while keeping the objective in \eqref{eq:PBA_REDUCED_OPT} constant, contradicting the optimality assumption of $\left \lbrace \distortion_i^* \right \rbrace$.
\end{proof}

There is at most one $\distortion_i^*$ such that $\distortion_i^* = \frac{\sigma_i^2}{2(\scalePBA -1)}\left( 1 + c_i\right)$. Assuming such an $i$ exists, $x_i = \frac{2(\scalePBA -1)}{1+c_i} < 2(\scalePBA -1)$. For the convex roots, $x_i = \frac{2(\scalePBA -1)}{1-c_i} > 2(a-1)$. Therefore from Lemma~\ref{lem:NORM_INC}, all the convex roots are contiguous. Therefore, the set of potentially optimal solutions reduces to cardinality $2d$, where each solution is characterized by the number of components that send non-zero rate and whether or not a concave root is sent. PBA, detailed in Algorithm~\ref{alg:PBA} finds the minimum value of the Lagrangian across these $2d$ solutions for a fixed $\lambda$. 
%Since the global optimal solution lies in these $2d$ solutions, PBA finds the global optimal solution to (\ref{eq:PBA_OPT_LAGRANGE}).
\end{proof}

Note that by sweeping $\lambda > 0$, one can compute the lower convex envelope of the $(D,R)$ curve.
Since every Pareto optimal $(D,R)$ must be a stationary point of (\ref{eq:PBA_OPT_LAGRANGE}),
one can also use Algorithm~\ref{alg:PBA} to compute the $(D,R)$ curve itself by sweeping $\lambda$
and retaining all those stationary points that are not Pareto dominated.




==> pba-tex 2/proofs_opti.tex <==
%\section{Proofs from Section~\ref{sec:PBA}} \label{sec:pfsPBA}
%
%\begin{proof}[Proof of Lemma~\ref{lem:WKdiagonal}]
% 
%From \eqref{eq:rewriteopti}, when $\encnew$ and $\cov$ are diagonal matrices, 
%\begin{equation}\label{eq:Tstruc}
%\decnew^* =
%  \begin{bmatrix}
%    \frac{\sigma_1^2 w_1}{1+\sigma_1^2 w_1^2} & & \\
%    & \ddots & \\
%    & & \frac{\sigma_d^2 w_d}{1+\sigma_d^2 w_d^2}.
%  \end{bmatrix}
%\end{equation}
%Substituting $\decnew^*$ from \eqref{eq:Tstruc} in \eqref{eq:rewriteopti} we have
%\begin{equation} \label{eq:rewritediagopti}
%\begin{aligned} 
%\min\limits_{\left \lbrace w_i \right \rbrace} \quad & \sum\limits_{i=1}^{d} \frac{\sigma_{i}^{2}}{1+w_{i}^{2} \sigma_{i}^{2}} \\
%\text{s.t.} \quad & R \geq \sum\limits_{i=1}^{d} \log(w_i^2 \sigma_i^2+1).
%\end{aligned}
%\end{equation}
%%It can be verified that if $\left \lbrace a_i \right \rbrace \geq 0$, $\frac{\partial^2}{\partial \lambda^2} (-\sum\limits_{i=1}^{d} \frac{(w_{i} + \lambda a_i)^{2} \sigma_{i}^{4}}{1+(w_{i} + \lambda a_i))^{2} \sigma_{i}^{2}}) \geq 0$ and $\frac{\partial^2}{\partial \lambda^2} (\sum\limits_{i=1}^{d} \log((w_i + \lambda a_i)^2 \sigma_i^2)) \geq 0$ at $\lambda=0$. This implies that the optimization problem is convex and since an interior point can be found in the feasible region, Slater's conditions hold, implying strong duality.
%
%Substituting $D_i = \frac{\sigma_i^2}{1+w_i^2 \sigma_i^2}$, we can convert this into a convex optimization problem.
%
%\begin{equation}
%\begin{aligned} 
%\min\limits_{\left \lbrace D_i \right \rbrace} \quad & \sum\limits_{i=1}^{d} D_i \\
%\text{s.t.} \quad & R \geq \sum\limits_{i=1}^{d} \log\left(\frac{\sigma_i^2}{D_i}\right)\\
%&D_i \leq \sigma_i^2
%\end{aligned}
%\end{equation}
%The Lagrangian can be written as 
%\[ \cL(\left \lbrace D_i, \mu_i \right \rbrace, \lambda)  = \sum\limits_{i=1}^{d} D_i + \lambda \left(\sum\limits_{i=1}^{d} \log\left(\frac{\sigma_i^2}{D_i}\right) - R \right) + \sum\limits_{i=1}^{d} \mu_i (D_i  - \sigma_i^2) \]
%The KKT conditions give us that 
%\[ \frac{\partial \cL}{\partial D_i} = 1 - \frac{\lambda}{D_i} + \mu_i = 0 \hspace{5mm} \forall i \in [d] \]
%Also we have $\lambda \geq 0, \mu_i \geq 0,  i \in [d]$ along with the complementary slackness conditions. When the rate constraint is not met with equality, $\lambda =0$ implying that $\mu_i = 0 $ $ \forall i \in [d]$, in turn implying that the distortions $D_i = \sigma_i^2$ $\forall i \in [d]$.
%
%Now, assume that the rate constraint is met with equality. Let $\cF = \left \lbrace i \in [d] \text{s.t. } \mu_i > 0 \right \rbrace$. Therefore for $i \in [d]\setminus \cF$, $\mu_i = 0$, implying $D_i = \lambda$. Note that for $i \in \cF$,  $D_i = \sigma_i^2$. Since the rate constraint is met with equality, it follows that 
%\[ e^R = \frac{\prod\limits_{i \in [d]\setminus \cF} \sigma_i^2}{D^{d-|\cF|}} \]
%The only thing that remains is identifying $\cF$. Observe that for $i \in cF$, 
%\[ \lambda = \sigma_i^2(1+\mu_i) > D_i = \sigma_i^2\]
%But we know that $\min_{i \in [d]\setminus \cF} \sigma_i^2 > \lambda > \max_{i \in \cF} \sigma_i^2$. 
%Therefore, $\cF$ consists of all indices whose variance is less than the common distortion $\lambda$.
%
%Therefore, for $1\leq s \leq d-1 $ when 
%\[ \sigma_s^2 \geq \left( \frac{\prod\limits_{i=1}^{s} \sigma_i^2}{e^R} \right)^{1/s} \geq \sigma_{s+1}^2 \] 
%or equivalently
%\[ \frac{\prod\limits_{i=1}^{s-1} \sigma_i^2 }{\sigma_s^{2s-2}} \leq e^R < \frac{\prod\limits_{i=1}^{s} \sigma_i^2 }{\sigma_{s+1}^{2s}}\] 
%we send $s$ components corresponding to the top $s$ variances ($\sigma_i^2$) with equal distortion and for the remaining $d-s$ components, the distortion is equal to the respective variances, $D_i = \sigma_i^2$.
%%\[ D_1 = D_2 \cdots D_d = \lambda, \]
%%\[  \prod_{i=1}^{d} D_i = e^{-R} \prod_{i=1}^{D} \sigma_i^2 \]
%%Therefore, distortions across components are equalized and equal to $e^{-R/d}  (\prod_{i=1}^{D} \sigma_i^2)^{1/d} $ and 
%%\[ w_i^2 = \frac{1}{D_i} - \frac{1}{\sigma_i^2} = e^{R/d}  (\prod_{i=1}^{D} \sigma_i^2)^{-1/d} - \frac{1}{\sigma_i^2} \]
%%Solving for the KKT conditions gives 
%%\begin{align*}\label{eq:kkt}
%%\lagmlt &= \frac{\sigma_i^4 w_i^2}{(1+\sigma_i^2 w_i^2)^2} \hspace{15mm} \forall i \in \left[ d \right]. \\
%%R &= \sum\limits_{i=1}^{d}  \log(w_i^2 \sigma_i^2).
%%\end{align*}
%%Therefore the rate constraint is met with equality. Also note that, the lagrange multiplier $\lagmlt$ is exactly equal to the absolute value of distortion across each component and is therefore the same for each component.
%\end{proof}
%
%
%
%%\begin{proof}[Proof of Lemma~\ref{lem:iterativetwodim}]
%%\textbf{First Direction}: 
%%
%%W.L.O.G assume that $\sigma_1 > \sigma_2$. We first find the single optimal direction, given that no signal is sent in the other directions. We write $\encnew$ as follows
%%\begin{equation}
%%\encnew = 
%%\begin{bmatrix}
%%   w_{11} & 0  \\
%%   w_{21} & 0
%%  \end{bmatrix}.
%%\end{equation}
%%Using the formulation in \eqref{eq:rewriteopti_inverse}, we can write the objective as follows. Note that the constraint is not the same as that in \eqref{eq:rewriteopti_inverse} since because of the zero signal directions, the problem would essentially be unconstrained.
%%\begin{equation}
%%\begin{aligned} 
%%\min\limits_{w_{11},w_{21}} \quad & \frac{\sigma_1^2 \sigma_2^2 \left( w_{11}^2 + w_{21}^2 \right) + \sigma_1^2 + \sigma_2^2 }{1 + \sigma_1^2 w_{11}^2 + \sigma_2^2 w_{21}^2} \\
%%\text{s.t.} \quad & R \geq  \log(\sigma_1^2 w_{11}^2 + \sigma_2^2 w_{21}^2).
%%\end{aligned}
%%\end{equation}
%%
%%Although the above optimization problem can be shown to be non-convex, we can derive some simple insights. First, lets assume that the constraint is satisfied. Therefore, 
%%\begin{equation*}
%%e^R = \sigma_1^2 w_{11}^2 + \sigma_2^2 w_{21}^2.
%%\end{equation*}
%%The above equation is an ellipse in two dimensions with the minor axes of length $\frac{e^{R/2}}{\sigma_1}$ and major axes of length $\frac{e^{R/2}}{\sigma_2}$. We plug the above equation in the objective function and observe that the optimal solution over this two dimensional ellipse is the least norm solution which is $w_{11} = \frac{e^{R/2}}{\sigma_1}, w_{21}=0$ and the value of the objective is $\sigma_2^2 + \frac{\sigma_1^2}{1+e^R}$.
%%
%%When the constraint is not satisfied, assume that for $0 < \delta \leq R$,
%%\begin{equation*}
%%e^{R-\delta} = \sigma_1^2 w_{11}^2 + \sigma_2^2 w_{21}^2.
%%\end{equation*}
%%We perform the same analysis as above and observe that over the above ellipse, the least norm solution is $w_{11} = \frac{e^{(R-\delta)/2}}{\sigma_1}$, $w_{21} = 0$. However, note that the objective is larger for this solution. Therefore, $w_{11} = \frac{e^{R/2}}{\sigma_1}, w_{21}=0$ is the optimal solution.
%%
%%\textbf{Second Direction}
%%
%%Given the above direction, we now find the second direction to send signal in. Since the rate constraint is now different, we don't fix the strength of the first direction to $\frac{e^{R/2}}{\sigma_1}$. We write $\encnew$ as follows 
%%
%%\begin{equation}
%%\encnew = 
%%\begin{bmatrix}
%%    a/ \sigma_1 & \encv[1]{2}  \\
%%   0 & \encv[2]{2}
%%  \end{bmatrix}.
%%\end{equation}
%%
%%Using the formulation in \eqref{eq:rewriteopti}, we can write the objective and the constraint as follows. 
%%
%%\begin{equation}
%%\begin{aligned} 
%%\max\limits_{a,\encv[1]{2}, \encv[2]{2} } \quad & \frac{a^2\sigma_1^2 \sigma_2^2 \encv[2]{2}^2 + a^2\sigma_2^4 \encv[2]{2}^2 + \sigma_1^4 \encv[1]{2}^2 + \sigma_2^4\encv[2]{2}^2 }{a^2 + 1 + \sigma_1^2 \encv[1]{2}^2 + (1+a^2) \sigma_2^2 \encv[2]{2}^2} \\
%%\text{s.t.} \quad & R \geq \log(a^2) +  \log(\sigma_1^2 \encv[1]{2}^2 + \sigma_2^2 \encv[2]{2}^2).
%%\end{aligned}
%%\end{equation}
%%To maximize the above equation w.r.t $a$, it can be proved that the inequality constraint has to be an equality. To see this note that the objective is a montone function of $a$ and the constraint forces $a^2$ to be between $0$ and $\frac{e^R}{\sigma_1^2 \encv[1]{2}^2 + \sigma_2^2 \encv[2]{2}^2}$ and it can be shown that the maximum is obtained when the inequality constraint is an equality.
%%
%%Let $\sigpr = \sigma_1/(\sqrt{a^2+1}), \rotencv[1]{2} = \encv[1]{2} \sigpr, \rotencv[2]{2} = \encv[2]{2} \sigma_2$. Rearranging the terms above, we obtain the following equivalent optimization problem 
%%
%%\begin{equation}\label{eq:twodimiterative}
%%\begin{aligned} 
%%\max\limits_{\rotencv[1]{2}, \rotencv[2]{2} } \quad & \frac{\sigpr^2\rotencv[1]{2}^2 + \sigma_2^2 \rotencv[2]{2}^2}{ 1 + \rotencv[1]{2}^2 + \rotencv[2]{2}^2} \\
%%\text{s.t.} \quad & \frac{e^R}{a^2} = (1+a^2) \rotencv[1]{2}^2 + \rotencv[2]{2}^2.
%%\end{aligned}
%%\end{equation}
%%
%%The constraint is an equation of an ellipse with minor axes $\frac{e^{R/2}}{\sqrt{a^2(1+a^2)}}$ and $\frac{e^{R/2}}{a}$. We now consider a circle of radius $\frac{e^{R/2}}{a} \gamma$, where $\gamma^2 \in \left[ \frac{1}{a^2+1}, 1 \right]$. We compute the objective at the intersection of the constraint ellipse and the above circle and express it as a function of $\gamma$. 
%%\begin{equation}
%%f(\gamma^2) = \frac{\sigpr^2\frac{e^R}{a^4}\left(1-\gamma^2\right)) + \sigma_2^2 \left(\frac{e^R}{a^2} \left(\gamma^2 - \frac{1-\gamma^2}{a^2} \right)\right)}{1+\frac{e^R}{a^2} \gamma^2}
%%\end{equation}
%%The above function can be shown to be monotone in $\gamma$. Therefore, the maximum is achieved at either $\gamma^2 = 1$ or $\gamma^2 = \frac{1}{a^2+1}$. We evaluate the objective at both these extreme points and pick the maximum value
%%
%%\begin{equation}
%%f\left(1\right) = \sigma_2^2 \frac{\frac{e^R}{a^2}}{1+\frac{e^R}{a^2}}, f\left(\frac{1}{a^2+1} \right) = \sigpr^2\frac{ \frac{e^R}{a^2 \left(1+a^2\right)}}{1 + \frac{e^R}{a^2 \left(1+a^2\right)}}
%%\end{equation}
%%
%%\end{proof}
%%
%%\begin{proof}[Proof of Lemma~\ref{lem:iterativegendim}]
%%W.L.O.G assume that $\sigma_1 \geq \sigma_2 \cdots  \geq \sigma_d$. Using the formulation in \eqref{eq:rewriteopti} we observe that the objective function can be written as 
%%\begin{equation}
%%\begin{aligned} 
%%\max\limits_{\encv{1}} \quad & \frac{\sum\limits_{j=1}^{d} \encv[j]{1}^2 \sigma_j^4}{1 + \sum\limits_{j=1}^{d} \encv[j]{1}^2 \sigma_j^2} \\
%%\text{s.t.} \quad & R \geq  \log(\sum\limits_{j=1}^{d} \encv[j]{1}^2 \sigma_j^2).
%%\end{aligned}
%%\end{equation}
%%Let $y_{j1} = \encv[j]{1} \sigma_j$. The above optimization problem can then be written as 
%%\begin{equation}
%%\begin{aligned} 
%%\max\limits_{y_1} \quad & \frac{\sum\limits_{j=1}^{d} y_{j1}^2 \sigma_j^2}{1 + \sum\limits_{j=1}^{d} y_{j1}^2 } \\
%%\text{s.t.} \quad & e^R \geq \sum\limits_{j=1}^{d} y_{j1}^2.
%%\end{aligned}
%%\end{equation}
%%Assume that the constraint is satisfied. The numerator of the objective describes an ellipsoid in $d$ dimensions and the constraint specifies a sphere of radius $e^{R/2}$. The largest such ellipsoid such that it just encompasses the constraint sphere is such that the smallest minor axis (which corresponds to the component with maximum variance i.e. $\sigma_1$) which implies that the rest of the components are 0 and $\encv[1]{1} = \frac{e^{R/2}}{\sigma_1}$. 
%%\end{proof}

==> pba-tex 2/questions.tex <==
%\section{Conclusion}
%In this work we model the task of compression as a linear autoencoder that quantizes the output of the encoder under rate constraints. We proved that for Schur-concave rate constraints, the optimal solution is to project data points along the eigenvectors. We recovered Principal Components Analysis (PCA) as a special case of this general formulation and we for a rate constraint function more attuned to compression, we proposed a waterfilling algorithm called Principal Bit Analysis (PBA). We studied a generalization called the Principal Bit-Components Analysis (PBCA) that recovers both PCA and PBA as its extreme cases and improves upon PBA's performance. We empirically verified that PBA improves on PCA for image datasets like MNIST, CIFAR-10 and the Faces Dataset. We also observed that PBA in fact improves upon JPEG and is comparable to JPEG2000, which are state-of-the art lossy compression algorithm optimized for images. We also observed a similar behaviour on an FSDD which is an audio dataset. 



==> pba-tex 2/related.tex <==
%\subsection{Related Work}

\textbf{Related Work.} Several recent works have examined how linear autoencoders can be 
modified to guarantee recovery of PCA. Most solutions involve eliminating the invariant global optimal solutions by introducing regularization of some kind. \cite{OftadehSWS20} propose a loss function which adds $k$ penalties to recover the $k$ principal directions, each corresponding to recovering up to the first $i \leq k$ principal directions. \cite{KuninBGS19} show that $\ell_2$ regularization helps reduce the symmetry group to the orthogonal group. \cite{BaoLSG20} further break the symmetry by considering non-uniform $\ell_2$ regularization and deterministic dropout. \cite{LadjalNP19} consider a nonlinear autoencoder with a covariance loss term to encourage finding orthogonal directions. Recovering PCA is an important problem even in the stochastic counterpart of autoencoders. \cite{LucasTGN19} analyze linear variational autoencoders (VAEs) and show that the global optimum of its objective is identical to the global optimum of log marginal likelihood of probabilistic PCA (pPCA). \cite{RolinekZM19} analyze an approximation to the VAE loss function and show that the linear approximation to the decoder is orthogonal. 

Our result on variable-rate compressors is connected to the sizable recent
literature on compression using autoencoder-like architectures. Representative 
contributions to the literature were noted above. Those works focus mostly
on the empirical performance of deep, nonlinear networks, with a particular
emphasis on finding a differentiable proxy for quantization so as to train
with stochastic gradient descent. In contrast, this work considers provable
properties of the compressors when trained perfectly.

%In recent years learning-based compressors have received significant interest. These are predominantly variable-rate, and they typically obtain the rate-distortion trade-off by training deep neural network-based autoencoders to minimize a rate-distortion lagrangian function \cite{TschannenAL18}, \cite{TodericiVJHMSC17}, \cite{BalleLS16}, \cite{TodericiOHVMBCS16}, \cite{TheisSCH17}, \cite{RippelB17}, \cite{HabibianRTC19}. The coded representation at the bottleneck layer of these autoencoders is further quantized \cite{AgustssonMTCTBG17} and entropy coded. Most of the challenge lies in figuring out a differentiable proxy for quantization so as to backpropagate through the autoencoders. \cite{BalleMSHJ18}, \cite{ZhouCGSW18} leverage the representation learning capability offered by latent variable models such as Variational Autoencoders (VAEs) for lossy compression. Instead of using standard distortion metrics like Peak Signal-To-Noise Ratio (PSNR), Mutli-scale Structural Similarity Index (MS-SSIM) \cite{AgustssonTMTG19} use Generative Adversarial Networks (GANs) to also minimize an adversarial loss that permits a lower distortion at low bit-rates. 

%Recent advances in generative models have enabled improved modeling of real-world high dimensional sources. It is well known that an accurate estimate of the source distribution results in a good lossless compression algorithm for the source. Using this principle, a recent line of work \cite{TownsendBB19}, \cite{HoogeboomPVW19}, \cite{HoLA19} modified the bits back coding scheme to be practically feasible with latent variable and flow-based generative models. For lossless text compression, Recurrent Neural Network (RNN) based models have been used in conjunction with entropy coding methods \cite{Mahoney00}, \cite{GoyalTCO19}. 





%Primarily efforts have been focused on improving upon state-of-the-art, non-learning based compression methods and on model compression. The former have leveraged advances in deep neural network architechtures 

%"Learned lossy compression"  - 
%<Para 1> - Works on compressing datasets. Bits-Back models source distribution to get lossless compression algorithms 

%<Para2 > - Lossy compression algorithms that are based on learning - Our work is not based on that. We don't learn anything here.

%Autoencoder - Unregularized autoencoder does not recover principal directions because of invertibility issues - Baldi and Hornik. Kunin showed L2--regularized autoencoders recover principal directions


==> pba-tex 2/schur.tex <==
\section{Review of Schur-Convexity}\label{app:schur}
    
  In this section, we review the key definitions and theorems related to Schur-convexity that we use in the proof of Theorem~\ref{thm:diagisoptimal}. 
  
  \begin{definition}{(\textbf{Majorization})}\cite{HornJ85}
For a vector $\bm{v} \in \RR^d$, let $\bm{v}^{\downarrow}$ denote the vector with the same components arranged in descending order. Given vectors $\bm{a}, \bm{b} \in \RR^{\ipdim}$, we say $\bm{a}$ majorizes $\bm{b}$ and denote $\bm{a} \succ \bm{b}$, if 
\[\sum\limits_{i=1}^{d} \left[\bm{a} \right]_i = \sum\limits_{i=1}^{d} \left[\bm{b} \right]_i,  \]
and for  all $k \in \left[ d-1 \right]$,
\[ \sum\limits_{i=1}^{k} \left[\bm{a}^{\downarrow} \right]_i \geq \sum\limits_{i=1}^{k} \left[\bm{b}^{\downarrow} \right]_i.\]

  \end{definition}

\begin{definition}{(\textbf{Schur-convexity})}
A function $f: \RR^{\ipdim} \rightarrow \RR$ is Schur-convex if for any vectors $\bm{a}, \bm{b} \in \RR^d$, such that $\bm{a} \succ \bm{b}$, 
\[ f\left( \bm{a} \right) \geq f\left( \bm{b} \right). \]
$f$ is strictly Schur-convex if the above inequality is a strict inequality for any $\bm{a} \succ \bm{b}$ that are not permutations of each other. $f$ is Schur-concave if the direction of the inequality is reversed and is strictly Schur concave if the direction of the inequality is reversed and it is a strict inequality for any $\bm{a} \succ \bm{b}$ that are not permutations of each other.
\end{definition}

\begin{proposition}\cite{MarshallOA11}\label{prop:single-letter}
If $f:\RR \rightarrow \RR$ is convex, then $\phi:\RR^d \rightarrow \RR$ given by
\[ \phi\left( \bm{v} \right) = \sum\limits_{i=1}^{d} f\left(\left[v \right]_i \right) \] 
is Schur-convex. If $f$ is concave, then $\phi$ is Schur-concave. Likewise if $f$ is strictly convex, $\phi$ is strictly Schur-convex and if $f$ is strictly concave, $\phi$ is strictly Schur-concave.
\end{proposition}


==> pba-tex 2/variable.tex <==
\section{Application to Variable-Rate Compression}\label{sec:VARIABLE}

We have seen that an autoencoder formulation inspired by 
data compression succeeds in providing guaranteed
recovery the principal source components. Conversely, 
a number of successful multimedia compressors have recently
been proposed that are either related to, or directly
inspired by, autoencoders~\cite{TschannenAL18, TodericiVJHMSC17,
BalleLS16, TodericiOHVMBCS16, TheisSCH17, RippelB17, HabibianRTC19,
AgustssonMTCTBG17, BalleMSHJ18, ZhouCGSW18, AgustssonTMTG19, BalleCMSJAHT20}.
In particular, Ball\'{e} \emph{et al.}~\cite{BalleMSHJ18}
show that the objective minimized by their compressor coincides with 
that of variational autoencoders. Following 
\cite{BalleCMSJAHT20}, we refer to this objective as \emph{nonlinear
transform coding (NTC)}. We next use Theorem~\ref{thm:diagisoptimal}
to show that
any minimizer of the NTC objective is guaranteed to recover
the principal source components if (1) the source is Gaussian,
 (2) the transforms are restricted to be linear,
and (3) the entropy model is \emph{factorized}, as explained below.

Let $\data \sim \cN\left(0,\cov\right)$, where $\cov$ is a positive semidefinite covariance matrix. As before, we consider an autoencoder defined by its encoder-decoder pair $(f,g)$, where for $k\leq d$, $f: \RR^{d} \rightarrow \RR^{k}$ and $g:\RR^{k} \rightarrow \RR^{d}$ are chosen from prespecified classes $\cC_f$ and $\cC_g$. The NTC framework
assumes dithered quantization during training, as in Section~\ref{sec:FRAMEWORK} and \cite{AgustssonT20, ChoiEL19}, and seeks to minimize the Lagrangian
\begin{equation}
\inf_{f \in \cC_f,g \in \cC_g} \mathbb{E}_{\data, \noise} \left[ \left \lVert \data - g\left( Q\left( f(\data) + \noise \right) - \noise \right) \right \rVert_2^2 \right] + \lambda H\left(Q \left( f( \data) + \noise\right) - \noise | \noise \right). 
\end{equation}
where $\lambda > 0$ and $\noise$ has i.i.d.\  $\text{Unif}\left[-0.5,0.5\right]$ components. 
NTC assumes variable-length compression, and the quantity
$$
H\left(Q \left( f( \data) + \noise\right) - \noise | \noise \right)
$$
is an accurate estimate of minimum expected codelength length for the discrete
random vector $Q \left( f( \data) + \noise\right)$.
As we noted in Section~\ref{sec:FRAMEWORK}, \cite{ZamirF92} showed that for any random variable $\data$, $Q\left( \data+ \noise \right) - \noise$ and $\data+\noise$ have the same joint distribution with $\data$. They also showed that $H\left(Q \left( \data + \noise\right) - \noise | \noise \right) = I\left( \data + \noise;\data \right) = h(\data + \noise)$, where
$h(\cdot)$ denotes differential entropy. Therefore, the objective can be written as
\begin{equation} \label{eq:general_lag}
 \inf_{f \in \cC_f,g \in \cC_g} \mathbb{E}_{\data, \noise} \left[ \left \lVert \data - g\left( f\left( \data \right) + \noise \right) \right \rVert_2^2 \right]  + \lambda h\left( f\left( \data \right) + \noise\right).
 \end{equation}
 (Compare eq.(13) in \cite{BalleCMSJAHT20}).

We consider the case in which $\cC_f, \cC_g$ are the class of linear functions. Let $\encnew, \decnew$ be $d$-by-$d$ matrices.  Define $f\left(\data\right) = \encnew^{\top} \data $, $g\left( \data \right) = \decnew \data$. Substituting this in the above equation, we obtain
\begin{equation}\label{eq:RD_LAG}
\inf\limits_{\encnew, \decnew} \mathbb{E}_{\data, \noise} \left[ \left \lVert \data - \decnew \left( \encnew^\top \data + \noise\right) \right \rVert_2^2 \right] \\ + \lambda h\left( \encnew^\top \data + \noise\right).
\end{equation}
Since $\decnew$ does not appear in the rate constraint, the optimal $\decnew$ can be chosen to be
the minimum mean squared error estimator of $\data \sim \cN\left( 0,\cov \right)$ given 
$\encnew^\top \data + \noise$, as in Section~\ref{sec:FRAMEWORK}. This gives
\begin{equation}\label{eq:RD_LAG_MMSE}
	\inf\limits_{\encnew} \tr(\cov) - \tr(\cov \encnew \left(\encnew^{\top} \cov \encnew + \frac{\ide}{12} \right)^{-1}\encnew^{\top} \cov ) + \lambda h\left( \encnew^\top \data + \noise\right).
\end{equation}

As noted earlier, the rate term $h\left( \encnew^\top \data + \noise\right)$ is an accurate 
estimate for the minimum expected length of the compressed representation of $Q \left( \encnew^\top \data+ 
\noise\right)$.
This assumes that the different components of this vector are encoded jointly, however. In
practice, one often encodes them separately, relying on the transform $\encnew$ to 
eliminate redundancy among the components. Accordingly, we replace the rate term with
$$
\sum_{i = 1}^d
h\left( \encvec_i^\top \data + [\noise]_i\right),
$$
%\begin{multline}\label{eq:RD_LAG_MMSE}
%\inf\limits_{\encnew} \tr(\cov) - \tr(\cov \encnew \left(\encnew^{\top} \cov \encnew + \frac{\ide}{12} \right)^{-1}\encnew^{\top} \cov ) \\ + \lambda I\left( \encnew^\top \data + \noise; \encnew^\top \data \right).
%\end{multline}
%For the remainder of the section we denote $ \tr(\cov) - \tr(\cov \encnew \left(\encnew^{\top} \cov \encnew + \frac{\ide}{ 12} \right)^{-1}\encnew^{\top} \cov )$ by $\text{MSE}\left( \cov, \encnew \right)$.
to arrive at the optimization problem
\begin{equation}\label{eq:RD_LAG_MMSE_FACTOR}
	\inf\limits_{\encnew} \tr(\cov) - \tr(\cov \encnew \left(\encnew^{\top} \cov \encnew + \frac{\ide}{12} \right)^{-1}\encnew^{\top} \cov )  + 
\lambda \cdot \sum_{i = 1}^d
h\left( \encvec_i^\top \data + [\noise]_i\right).
\end{equation}

\begin{theorem}
Suppose $\cov$ has distinct eigenvalues. 
	Then any $\encnew$ that achieves the infimum in~(\ref{eq:RD_LAG_MMSE_FACTOR}) 
 has the property that all of its nonzero rows are eigenvectors of $\cov$.
\label{thm:variable_rate}
\end{theorem}

\begin{proof}
Since the distribution of $\noise$ is fixed, by the Gaussian assumption on $\data$, 
$ h\left( \encvec_j^\top \data + [\noise]_j\right)$ only depends on
	$\encvec_j$ through $\encvec^{\top}_j \cov \encvec_j$. Thus we may write
	\begin{equation}
		h(\encvec_j^{\top} \data + \epsilon)
		    =  \rateproxy_{sl}(\encvec_j^{\top} \cov \encvec_j).
	\end{equation}
	By Theorem~\ref{thm:diagisoptimal}, it suffices to show that $\rateproxy_{sl}(\cdot)$
	is strictly concave.
	Let $Z$ be a standard Normal random variable and let $\epsilon$
      be uniformly distributed over $[-1/2,1/2]$, independent of $Z$. 
         Then we have
	\begin{align}
		\rateproxy_{sl}(s) 
		 & = h(\sqrt{s} \cdot Z + \epsilon).
	\end{align}
	Thus by de Bruijn's identity~\cite{CoverT06},
	\begin{equation}
		\rateproxy'_{sl}(s) = \frac{1}{2} J(\epsilon + \sqrt{s} \cdot Z),
	\end{equation}
	where $J(\cdot)$ is the Fisher information. To show that $\rateproxy'_{sl}(\cdot)$
	is strictly concave, it suffices to show that $J(\epsilon + \sqrt{s} \cdot Z)$ is strictly
	decreasing in $s$.\footnote{If $g'(\cdot)$ is strictly decreasing then for all $t > s$,
	$g(t) = g(s) + \int_s^t g'(u) du < g(s) + g'(s)(t-s)$ and likewise for $t < s$. 
	 That $g(\cdot)$ is strictly
	concave then follows from the standard first-order test for 
	concavity~\cite{BoydVandenberghe}.}
	To this end, let $t > s > 0$ and let $Z_1$ and $Z_2$ 
	  be i.i.d.\ standard Normal random variables, independent of $\epsilon$. Then
	  \begin{equation}
		   J(\epsilon + \sqrt{t} \cdot Z) = J(\epsilon + \sqrt{s}\cdot Z_1 + \sqrt{t-s}\cdot Z_2)
	  \end{equation}
	  and by the convolution inequality for Fisher information~\cite{Blachman65},
	  \begin{align}
\frac{1}{J(\epsilon + \sqrt{s} \cdot Z_1 + \sqrt{t - s} \cdot Z_2)}  >
		       \frac{1}{J(\epsilon + \sqrt{s} \cdot Z_1)} + \frac{1}{J(\sqrt{t-s} \cdot Z_2)}> \frac{1}{J(\epsilon + \sqrt{s} \cdot Z_1)},
	  \end{align}
      where the first inequality is strict because $\epsilon + \sqrt{s} \cdot Z_1$
       is not Gaussian distributed.
\end{proof}

%\begin{theorem}\label{thm:variable_rate}
%Let $\cov$ be a covariance matrix and $\lambda, D > 0$. Among all $\encnew$ with a fixed $\text{MSE}\left( \cov, \encnew \right) = D$, the $\encnew$ that minimizes \eqref{eq:RD_LAG_MMSE} is such that its rate is within 0.255 bits per dimension of the optimal rate for reconstructing a zero-mean Gaussian source with covariance matrix $\cov$, with distortion $D$.
%\end{theorem}
%\begin{proof}
%The least possible rate achievable by a fixed-rate compression scheme for a given distortion $D$ is given by the rate-distortion function of the Gaussian source with covariance matrix $\cov$ \cite{CoverT06}. Although our formulation in \eqref{eq:RD_LAG_MMSE} is for a variable-rate compression scheme, the rate term in the Lagrangian is averaged over source realizations. Therefore, the Gaussian rate-distortion function is a lower bound for the optimal rate in \eqref{eq:RD_LAG_MMSE} for a fixed distortion. 
%
%Let $\sigma^2 = \frac{1}{12}$. For the upper bound we have
%\begin{align*}
%I\left( \encnew^\top \data + \noise; \encnew^\top \data \right) &= h\left( \encnew^\top \data + \noise \right) - h\left( \noise \right) \\
%&= h\left( \encnew^\top \data + \noise \right)\\
%&\leq h\left( \encnew^\top \data + \noise_G \right)\\
%&= \frac{\ipdim}{2} \log \left( 2\pi e \right) + \frac{1}{2} \log \left \lvert \encnew^\top \cov \encnew + \sigma^2 \ide \right \rvert.
%\end{align*}
%The above expression is invariant to orthogonal transformations. Therefore, similar to the proof of Theorem~\ref{thm:diagisoptimal}, we can show that the optimal $\encnew$ is such that $\encnew^\top \cov \encnew$ is diagonal. This implies that 
%\begin{equation}
%\log \left \lvert \encnew^\top \cov \encnew +  \sigma^2 \ide \right \rvert = \sum\limits_{j=1}^{d} \log \left( \encvec_j^\top \cov \encvec_j + \sigma^2 \right).
%\end{equation}
%
%Therefore \eqref{eq:RD_LAG_MMSE} can be upper bounded as 
%\begin{equation}\label{eq:RD_LAG_UB}
%\inf\limits_{\encnew: \encnew^\top \cov \encnew \text{ is diagonal} } \text{MSE}\left( \cov, \encnew\right) + \lambda \left( \frac{\ipdim}{2} \log \left( 2\pi e \right) + \frac{1}{2}  \sum\limits_{j=1}^{d} \log \left( \encvec_j^\top \cov \encvec_j + \sigma^2 \right) \right).
%\end{equation}
%
%Ignoring the constant $\frac{\lambda d \log\left( 2\pi e \right)}{2}$, the rest of the expression in \eqref{eq:RD_LAG_UB} is the Lagrangian of the constrained rate-distortion formulation in \eqref{eq:MASTEROPTI_MMSE} where the constraint is Schur-concave. Therefore by Theorem~\ref{thm:diagisoptimal}, $\encnew$'s nonzero columns are eigenvectors of $\cov$. Therefore, \eqref{eq:RD_LAG_UB} reduces to 
%\begin{equation}\label{eq:RD_LAG_UB_diag}
%\inf\limits_{\left \lbrace \scaling_i \right \rbrace} \sum\limits_{i=1}^{d} \frac{\sigma_{i}^{2}}{1+\scaling_{i}^{2} \frac{\sigma_{i}^{2}}{\sigma^2}} + \lambda \left( \frac{\ipdim}{2} \log \left( 2\pi e \sigma^2 \right) + \frac{1}{2}  \sum\limits_{j=1}^{d} \log \left( \scaling_j^2 \frac{\sigma_j^2}{\sigma^2} + 1\right) \right).
%\end{equation}
%Apart from the constant term of $\frac{\lambda \ipdim \log\left(2\pi e \sigma^2 \right)	}{2} \sim 0.255\lambda \ipdim$, the Lagrangian above is the same as the Lagrangian of PBA with $\scalePBA=1$. This implies that the upper bound on the rate for the Lagrangian\eqref{eq:RD_LAG_MMSE} is given by the Gaussian rate-distortion function plus a constant that is within 0.255 bits per dimension. 
%\end{proof}

%Theorem~\ref{thm:variable_rate} shows that, for a fixed distortion $D>0$, there exists a variable-rate linear autoencoder based compressor that can achieve the optimal rate for a Gaussian source within $0.255$ bits per dimension. Since the class of neural networks subsumes linear functions, for a fixed distortion $D>0$, the minimizing $f,g$ for \eqref{eq:general_lag} is such that its rate is within $0.255$ bits per dimension of the optimal rate for a Gaussian source.

